Disentangling Noise from Images: A Flow-Based Image Denoising Neural Network

The prevalent convolutional neural network (CNN) based image denoising methods extract features of images to restore the clean ground truth, achieving high denoising accuracy. However, these methods may ignore the underlying distribution of clean images, inducing distortions or artifacts in denoising results. This paper proposes a new perspective to treat image denoising as a distribution learning and disentangling task. Since the noisy image distribution can be viewed as a joint distribution of clean images and noise, the denoised images can be obtained via manipulating the latent representations to the clean counterpart. This paper also provides a distribution learning based denoising framework. Following this framework, we present an invertible denoising network, FDN, without any assumptions on either clean or noise distributions, as well as a distribution disentanglement method. FDN learns the distribution of noisy images, which is different from the previous CNN based discriminative mapping. Experimental results demonstrate FDN's capacity to remove synthetic additive white Gaussian noise (AWGN) on both category-specific and remote sensing images. Furthermore, the performance of FDN surpasses that of previously published methods in real image denoising with fewer parameters and faster speed. Our code is available at: https://github.com/Yang-Liu1082/FDN.git.

==> secs/BackGround.tex <==
% \begin{comment}
% We obtained our latent representations using Glow~\cite{Glow}(normalizing flow architecture), which can learn complex distributions accurately without any information loss. In this section, we introduce the related background of the aforementioned architecture.
% \end{comment}

% \begin{comment}
% \subsection{Choosing Proper Generative Models for \\Image Denoising}
% As we have described in the introduction part, the traditional view of image denoising networks as discriminative models cannot allow us to utilize our prior knowledge about the distributions of the given data. As a result, discriminative models are more data-consuming and are prone to overfitting. The limitations of discriminative models motivate us to consider image denoising networks as generative models, equipping us the capability of making assumptions of the given data. 

% To view image denoising networks from discriminative models as generative ones, we require the generative models for image denoising have two properties: (1) the models support estimating the probability densities of the given data; (2) the models map an image to a single latent representation in a one to one fashion. The first property allows making assumptions of the given data, and the second property facilitates removing noises form the representation, followed by reconstructing a clean image from the noise-removed representation. 

% However, the two required properties for viewing generative models as image denoising networks are not aligned with the common requirements for building generative models. Standard generative models do not demand the one-to-one mapping between the input and the latent representation. For example, judged from citations, two mainstream generative models are variational autoencoders (VAEs) and generative adversarial networks (GANs); however, neither VAEs nor GANs map an input image to a unique latent representation. As a result, we resort to a more recently proposed generative models that are gaining increasing attention: the flow-based generative models. 
% \end{comment}


% Our latent representations are got by Glow~\cite{Glow}, a kind of normalising flow architecture, which can learn complex distributions accurately without any information loss. 
% In this section, we introduce some related background of this architecture.

% \begin{comment}
% \subsection{Normalizing Flows}
% Normalizing flow, first proposed by Dinh~\cite{NICE}, is a tool for computing complex posterior distribution accurately by applying a sequence of invertible transformations through easily computable Jacobians to a simple base distribution, transforming it into a complex distribution. 

% % Normalising flow is a tool to calculate complex posterior distribution accurately.
% % % is a sequence composed of several applications of the change of variables formula~\cite{Deco_NF}. 
% % It was first proposed by Dinh in 2014~\cite{NICE}. They applied a sequence of invertible transformations with easily computable Jacobians to a simple base distribution, to transform it to a complex distribution. 

% %\SA{I am here}
% Assume \textbf{z} is a random variable and $\textbf{z} \sim q(\textbf{z})$. Further, $f:\mathbb{R}^D \rightarrow \mathbb{R}^D$ is an invertible mapping, which transforms \textbf{z} to another random variable $\textbf{z}^{'} = f(\textbf{z})$. 
% \SA{you mean another random variable}. \LY{Yes.}
% The density of $\textbf{z}^{'} \sim q(\textbf{z}^{'})$ can be achieved through the following equation

% % Assume \textbf{z} is a random variable and $\textbf{z} \sim q(\textbf{z})$. $f:\mathbb{R}^D \rightarrow \mathbb{R}^D$ is an invertible mapping, 
% % % with $f^{-1} = g$ as inverse, i.e., $g \circ f(\textbf{z}) = \textbf{z}$,
% % which transforms \textbf{z} to a random variable $\textbf{z}^{'} = f(\textbf{z})$. The density of $\textbf{z}^{'} \sim q(\textbf{z}^{'})$ can be achieved through the following equation

% \begin{equation}
% \begin{split}
%         q(\textbf{z}^{'}) &=q(\textbf{z})\big|\det(\frac{\partial f^{-1}(\textbf{z}^{'})}{\partial \textbf{z}^{'}})\big|\\
%         &=q(\textbf{z})\big|\det(\frac{\partial f(\textbf{z})}{\partial \textbf{z}})\big|^{-1}.
% \end{split}
% \label{Eq:density}
% \end{equation}

% By composing several simple transformations $f$ as shown in Eq~\ref{Eq:density}, we obtain arbitrarily complex density $q(\textbf{z}^{'})$ from a simple base distribution $q(\textbf{z})$. We denote $\textbf{z}_{K}$ as the random variable obtained by successively transforming a random variable $\textbf{z}_0$.
% % By composing several this kind of simple transformations $f$, we can get arbitrarily complex density $q(\textbf{z}^{'})$ from a simple base distribution $q(\textbf{z})$. We denote $\textbf{z}_{K}$ as the random variable obtained by successively transforming a random variable $\textbf{z}_0$.

% \begin{equation}
%     \textbf{z}_{K} = f_{K}\circ ... \circ f_{2} \circ f_{1}(\textbf{z}_0).
% \end{equation}

% The log density of $q_{k}(\textbf{z}_{K})$ can be calculated as:

% \begin{equation}
%     \log q_{k}(\textbf{z}_{K}) = \log q_{0}(\textbf{z}_{0})-\sum_{k=1}^{K} \log \det|\frac{\partial \textbf{f}_{k}}{\partial \textbf{z}_{k}}|
% \end{equation}

% We can train the normalizing flow to estimate very complex distributions by maximizing the log-likelihood $\log q_{k}(\textbf{z}_{K})$. However, the estimation of Jacobian is an expensive operation (\ie $\mathcal{O}(D^3)$); therefore, to achieve computational efficiency, transformations with a triangular Jacobian matrix are chosen. \SA{Check the accuracy of the last sentence}\LY{It's correct.}
% \end{comment}

% By maximizing the log-likelihood $\log q_{k}(\textbf{z}_{K})$, we can train the normalising flow to estimate very complex distributions. However, the computation of Jacobian is $\mathcal{O}(D^3)$, which is usually improved by choosing transformations with a triangular Jacobian matrix to make the computation more efficient.

% Glow based image restoration. \SA{Not a good caption, please rephrase it and give a little bit information about squeeze, step of flow and split}

% \begin{comment}
% \subsection{Glow}
% Glow~\cite{Glow} is an excellent generative model based on normalizing flow, which extends NICE~\cite{NICE} and NVP~\cite{RealNVP} and demonstrates significant improvement on the generation quality of natural images. A Glow model mainly consists of three components, \ie Actnorm layers, Invertible $1\times1$ convolutional layers, and Affine Coupling layers. Moreover, Squeeze and Split layers are also employed to facilitate multi-scale learning.
% \end{comment}

% Glow~\cite{Glow} is an excellent generative model based on normalising flow, which extends NICE~\cite{NICE} and NVP~\cite{RealNVP} and demonstrates significant improvement on generation quality of natural images. A Glow model mainly consists of three kinds of components, i.e., Actnorm layers, Invertible $1\times1$ convolutional layers and Affine Coupling layers. Squeeze and Split layers are also employed to facilitate multi-scale learning.

% \textbf{Actnorm layers} are layers with scale and translation parameters, performing affine transformations of the activations, as illustrated in Equ.~\ref{Equ: Actnorm}. They are data-dependent initialized \SA{re-write} such that the post-actnorm activations per-channel has zero mean and unit variance. After initialization, they are trainable parameters during training \SA{re-write}. Actnorm layers improve training stability and performance.
% \begin{equation}\label{Equ: Actnorm}
%     \textbf{y} = \textbf{s} \odot \textbf{x} + \textbf{b},
% \end{equation}
% where the scale parameters $\textbf{s}$ and bias $\textbf{b}$ are $1\times c$ scalars. And $c$ is the number of channels.

% \textbf{Invertible $1\times1$ convolutional layers} are generalizations of permutation operations employed in NICE~\cite{NICE} and Real NVP~\cite{RealNVP}, which is represented in Equ.~\ref{Equ: Invertible}.

% \textbf{Invertible $1\times1$ convolutional layers} are generalizations of permutation operations employed in NICE~\cite{NICE} and Real NVP~\cite{RealNVP}, which is represented as Equ.~\ref{Equ: Invertible}.
% $1 \times 1$ Concolutions are easy to invert, and can be seen as a generalization of the permutation operations that were used by Dihn et al.~\cite{}. 
% $1 \times 1$ convolutions improve the effectiveness of the coupling layers.
% \begin{equation}\label{Equ: Invertible}
%     \textbf{y} = \textbf{W}\textbf{x},
% \end{equation}
% where $\textbf{W}$ is a $c \times c$ matrix.

% \textbf{Affine Coupling layers} capture the correlations among spatial dimensions, same as in NICE~\cite{NICE} and Real NVP~\cite{RealNVP}.
% Coupling layers~\cite{} split the input into two parts. The output is a combination of a copy of the first half, and a transformation of the second half, parametrized by the first part.
% \begin{equation}\label{Equ: Affine Coupling_1}
%     \textbf{x}_{a}, \textbf{x}_{b} = split(\textbf{x}), 
% \end{equation}
% \begin{equation}\label{Equ: Affine Coupling_2}
%     \textbf{s}_2, \textbf{b}_2 = NN(\textbf{x}_b),
% \end{equation}
% \begin{equation} \label{Equ: Affine Coupling_3}
%     \textbf{y}_{a} = \textbf{s}_2 \cdot \textbf{x}_{a}+ \textbf{b}_2, \textbf{y} = concat(\textbf{y}_a, \textbf{x}_b), \\    
% \end{equation}
% where $NN(\cdot)$ is a neural network, $split(\cdot)$ and $concat(\cdot)$ operates along channel dimension.

==> secs/Experiments_old.tex <==
\section{Experiment}
As the first distribution learning and disentanglement based method, the applications of \ourmodel are studied thoroughly in this paper. 
We apply \ourmodel to denoise category-specific images first. Since category-specific images usually have similar patterns in all the images, such as the facial contours and features in human faces, the distribution of them is easier to learn than random nature images.  
Then, the experiment is extended to denoising more difficult remote sensing images, which contains diverse terrain patterns, such as mountains or forests, following intricate distributions. At last, we investigate our capacity in removing noise which follows complicated  distribution in the real noise dataset.
Further details are provided about the datasets, training strategies and both qualitative and quantitative results in this section.

\subsection{Experimental Settings}
\subsubsection{Datasets}
\noindent
\textbf{Category-Specific datasets:} We investigate the capacity of \ourmodel in removing AWGN on three category-specific datasets, including face, flower, and bird images. 
\begin{itemize}
\item  CelebA~\cite{CelebA} is a large human face dataset, containing 202,599 face images. We use the 162770 training images for training and 19867 validation images for testing. The training images are cropped into $64 \times 64$ patches randomly as the input of the network at training stage. Since the training set is large enough, we do not apply any data augmentation during training. 
    
\item  Flower Dataset~\cite{Flower} contains 102 categories of flowers, including 1020 training images, 1020 validation images, and 6149 test images. To better learn the distribution of flowers, we change the partition of the dataset and use the 6149 images as the training set and the remaining 2040 images as the test set. The training images are randomly cropped into patches with a size of $128 \times 128$. Flipping and rotation are employed as data augmentation. 

\item  CUB-200 Dataset~\cite{Bird} includes 11,788 bird images, covering 200 categories of birds. We use 5989 images as the training set and 5790 images as the test set. The training images are cropped into $128 \times 128$ patches with randomly flipping as data augmentation during training.
\end{itemize}

\noindent
\textbf{Remote Sensing datasets:} 
We attempt to denoise two remote sensing datasets (RICE1 and RICE2~\cite{RICE}) with AWGN added to explore our capability when the ground truth images' distribution becomes complex. The datasets contain 500 and 450 pairs of images with a size of $512\times512$ separately. We randomly crop patches of size $64\times64$ from the images for training and add AWGN with $\sigma=30, 50$, and $70$ to get noise-free and noisy pairs, respectively. Random flipping as well as rotation are utilized for data augmentation.

\noindent
\textbf{Real Noisy datasets:}
Finally, we verify ~\ourmodel's effectiveness in removing real noise, which follows intricate distribution. Real image noise can result from photon shot noise, fixed pattern noise, dark current, readout noise, quantization noise and so on during the imaging process~\cite{Real_Noise_Source}. We conduct real noise removal on the dataset SIDD~\cite{SIDD_2018_CVPR}, which is taken by five smartphone cameras with small apertures and sensor sizes. The medium SIDD dataset contains 320 clean and noisy pairs. Patches with a size of $144 \times 144$ are randomly cropped for training. Flipping and rotation are adopted for augmentation.

\subsubsection{Training Details}
\ourmodel with 2 DownScale Flow blocks and 8 SoF blocks in each Flow blocks is exploited in our experiment, where Adam~\cite{kingma2014adam} is engaged as an optimizer. The learning rate is initialized as $2 \times 10^{-4}$ and halved after every 50K iterations. To evaluate the methods, we employ Peak Signal-to-Noise Ratio (PSNR) as the evaluation metrics.

\subsection{Ablation Study}
\textbf{Number of Flow and SoF Blocks.}
We study the denoising effects of employing different numbers of Flow and SoF blocks in~\ourmodel. We train models on CelebA~\cite{CelebA} with $\sigma=50$ AWGN added. The results on the 50Kth iteration on the validation set are reported in~\autoref{Tab:blocks}.
In general, given the same number of Flow blocks, the more SoF blocks in each of the Flow blocks, the higher the denoising accuracy. However, the improvement is not significant when we have 3 Flow blocks.
On the other hand, with the same number of SoF blocks in each Flow block, increasing Flow block numbers from 1 to 2 improves the performance. However, further increment results in similar accuracy when SoF=4 and even a little bit decrease when SoF=8. Thus, we adopt 2 Flow blocks with 8 SoF blocks contained in our experiment.

\begin{table}[]
\centering
\caption{Comparisons on the denoising accuracy of different numbers of DownScale Blocks and Invertible Blocks.}
% \resizebox{0.42\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\hline\hline
\multicolumn{2}{l|}{\multirow{2}{*}{PSNR}} & \multicolumn{2}{c}{SoF Blocks}                 \\ \cline{3-4} 
\multicolumn{2}{l|}{}& \multicolumn{1}{c|}{num = 4} & \multicolumn{1}{c}{num = 8} \\ \hline
\multirow{3}{*}{Flow Blocks} & num = 1 & 29.59 & 29.86 \\ \cline{2-4} 
& num = 2 & 29.87 & \textcolor{red}{30.00} \\ \cline{2-4} 
& num = 3 & 29.89 & 29.90 \\ \hline
\hline
\end{tabular}
% }
\label{Tab:blocks}
\end{table}

\begin{table}
\centering
\caption{Comparisons on different proportions of the dimensions of $\zc$ in $\z$.} 
\begin{tabular}{cccccc}
\hline
\hline
dim($\zc$) & 1/8 & 1/4 & 1/2 & 3/4 & 7/8 \\ 
\hline
 PSNR & 29.81 & 30.00 & 30.00 & \textcolor{red}{30.19} & 30.18 \\ \hline
\hline
\end{tabular}
\label{Tab:dim}
% \vspace{-4mm}
\end{table}

\begin{table*}[]
\centering
\caption{Comparisons of removing synthetic noise on three category-specific datasets. Our \ourmodel outperforms the other competitive methods on most of the three datasets for three different noise levels.} 
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline\hline
Dataset & $\sigma$ & BM3D~\cite{BM3D} & EPLL~\cite{EPLL} & IRCNN~\cite{IRCNN} & REDNet~\cite{REDNet} & DnCNN~\cite{DnCNN} & FFDNet~\cite{zhang2018ffdnet} & \ourmodel \\ \hline
& 15 & 35.46 & 33.29 & 35.20 & 35.23 & 35.04 & 35.14 & \textbf{35.74} \\
& 25 & 32.80 & 30.81 & 32.62 & 32.68 & 32.63 & 32.40 & \textbf{32.95} \\
& 50 & 29.46 & 27.65 & 29.24 & 29.56 & 29.57 & 29.44 & \textbf{30.29} \\ 
\multirow{-4}{*}{CelebA~\cite{CelebA}} & Blind & -- & -- & 31.92 & 33.16 & 32.17 & 32.20 & \textbf{33.52} \\ \hline
& 15 & 37.20 & 35.41 & 36.83 & 36.93 & 36.73 & 36.49 & \textbf{37.38} \\
& 25 & 34.73 & 32.92 & 34.47 & 34.75 & 34.17 & 33.89 & \textbf{34.82} \\
& 50 & 31.38 & 29.58 & 30.8 & 31.34 & 30.38 & 30.74 & \textbf{31.71} \\
\multirow{-4}{*}{Flower~\cite{Flower}} & Blind & -- & -- & 34.91 & 34.57 & 34.55 & 34.61 & \textbf{35.18}\\ \hline
& 15 & 35.08 & 33.31 & 35.14 & 35.16 & 35.21 & 34.86 & \textbf{35.30} \\
& 25 & 32.59 & 30.83 & 32.71 & 32.80 & 32.45 & 32.33 & \textbf{32.94} \\
& 50 & 29.32 & 27.61 & 29.28 & 29.72 & 28.87 & 28.61 & \textbf{29.79} \\
\multirow{-4}{*}{CUB-200~\cite{Bird}} & Blind & -- & -- & 32.49 & 33.18 & 32.89 & 33.07 & \textbf{33.20} \\\hline
\hline
\end{tabular}
\label{Tab:Class_Specific AWGN Denoise}
\end{table*}

\textbf{The split of $\zc$ and $\zn$.}
We also study the effects of different dimension numbers of $\zc$ (i.e., dim($\zc$)). Models are trained with dim($\zc$) = 1/8, 1/4, 1/2, 3/4 and 7/8 dim($\z$) separately and the validation results on the 50Kth iteration are reported in~\autoref{Tab:dim}. In general, the denoising accuracy improves with the increasing of the proportion of dim($\zc$). On the other hand, the results are almost the same when dim($\zc$) = 3/4 and 7/8 dim($\z$), illustrating that extending the dimensions of $\zc$ will not boost the denoising performance further. Thus, we use dim($\zc$) = 3/4 dim($\z$) in our experiment.

\subsection{Category-Specific Image Denoising}

\textbf{Quantitative Results.} 
In Table~\ref{Tab:Class_Specific AWGN Denoise}, we report numeric values for the three category-specific datasets added with AWGN with the level of $\sigma=15, 25$ and $50$. Compared with other competitive methods in synthetic noise removal, \ourmodel achieves the highest PSNR on all the datasets and noise levels. 

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{secs/images/Face.pdf}
% \vspace{-3cm}
\caption{The image denoising results of \ourmodel on CelebA with $\sigma=50$ against competitive methods.}
\label{fig:Visual_CelebA}
\end{figure*}

\begin{figure*}[ht]
\centering
% Bird 1
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_1/box_bird_gt_image_15.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_1/cropped_bird_S50.0_corrupted_image_15.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_1/cropped_bird_S50.0_DnCNN_denoised_image_15.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_1/cropped_bird_S50.0_FFDNet_denoised_image_15.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_1/cropped_bird_S50.0_dncnn_sk_conGradient_before_denoised_image_15.png}
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_1/cropped_bird_S50.0_glow_denoised_image_15.png}
\end{subfigure}

% Bird 2
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_2/box_bird_gt_image_46.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_2/cropped_bird_S50.0_corrupted_image_46.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_2/cropped_bird_S50.0_DnCNN_denoised_image_46.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_2/cropped_bird_S50.0_FFDNet_denoised_image_46.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_2/cropped_bird_S50.0_dncnn_sk_conGradient_before_denoised_image_46.png}
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_2/cropped_bird_S50.0_glow_denoised_image_46.png}
\end{subfigure}

% Bird 3
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_3/box_bird_gt_image_52.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_3/cropped_bird_S50.0_corrupted_image_52.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_3/cropped_bird_S50.0_DnCNN_denoised_image_52.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_3/cropped_bird_S50.0_FFDNet_denoised_image_52.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_3/cropped_bird_S50.0_dncnn_sk_conGradient_before_denoised_image_52.png}
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_3/cropped_bird_S50.0_glow_denoised_image_52.png}
\end{subfigure}

% Bird 4
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_4/box_bird_gt_image_56.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_4/cropped_bird_S50.0_corrupted_image_56.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_4/cropped_bird_S50.0_DnCNN_denoised_image_56.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_4/cropped_bird_S50.0_FFDNet_denoised_image_56.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_4/cropped_bird_S50.0_dncnn_sk_conGradient_before_denoised_image_56.png}
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_4/cropped_bird_S50.0_glow_denoised_image_56.png}
\end{subfigure}

% Caption
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \caption*{GT} 
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \caption*{Noisy} 
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \caption*{DnCNN} 
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \caption*{FFDNet}   
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \caption*{GradNet} 
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \caption*{\ourmodel} 
\end{subfigure}
\caption{The comparison of denoising results on CUB-200 with $\sigma=50$ AWGN.}
\label{fig:Visual_Bird}
\end{figure*}

% \SA{Remove UNET and use another method if possible, zoom in on the duck to show the artifacts.}

\begin{figure*}[ht]
\centering
% Flower one
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/flower_1/box_flower_gt_image_1.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_1/cropped_flower_S50.0_corrupted_image_1.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_1/cropped_flower_S50.0_DnCNN_denoised_image_1.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/flower_1/cropped_flower_S50.0_FFDNet_denoised_image_1.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_1/cropped_flower_S50.0_dncnn_sk_conGradient_before_denoised_image_1.png}
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_1/cropped_flower_S50.0_glow_denoised_image_1.png}
\end{subfigure}

% Flower 2
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/flower_2/box_flower_gt_image_17.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_2/cropped_flower_S50.0_corrupted_image_17.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_2/cropped_flower_S50.0_DnCNN_denoised_image_17.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/flower_2/cropped_flower_S50.0_FFDNet_denoised_image_17.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_2/cropped_flower_S50.0_dncnn_sk_conGradient_before_denoised_image_17.png}
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_2/cropped_flower_S50.0_glow_denoised_image_17.png}
\end{subfigure}

% Flower 3
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/flower_3/box_flower_gt_image_69.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_3/cropped_flower_S50.0_corrupted_image_69.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_3/cropped_flower_S50.0_DnCNN_denoised_image_69.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/flower_3/cropped_flower_S50.0_FFDNet_denoised_image_69.png}  
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_3/cropped_flower_S50.0_dncnn_sk_conGradient_before_denoised_image_69.png}
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/flower_3/cropped_flower_S50.0_glow_denoised_image_69.png}
\end{subfigure}

% Caption
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \caption*{GT} 
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \caption*{Noisy} 
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \caption*{DnCNN} 
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include first image
  \caption*{FFDNet}   
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \caption*{GradNet} 
\end{subfigure}
\begin{subfigure}{.13\textwidth}
  \centering
  % include second image
  \caption*{\ourmodel} 
\end{subfigure}

\caption{The comparisons on Flower for $\sigma=50$ against state-of-the-art methods. }
\label{fig:Visual_Flower}
\end{figure*}

We also employ the same \ourmodel for blind denoising with noise levels between [0, 55], as shown in~\autoref{Tab:Class_Specific AWGN Denoise}. The distribution of blind noise is Gaussian Mixture Model, which is much more complicated than the Gaussian distribution with a certain noise level. 
Although tradition methods such as BM3D~\cite{BM3D} and EPLL~\cite{EPLL} is good at removing Gaussian noise, their capacity in blind denoising is unavailable due to the requirement of noise level as input.
Comparing with other feature learning based CNN methods, \ourmodel outperforms others to a large extend in most of the cases, exhibiting our superiority in category-specific image denoising.

\textbf{Qualitative Results.} The visual results are shown in Figure~\ref{fig:Visual_CelebA}, ~\ref{fig:Visual_Bird} and ~\ref{fig:Visual_Flower}. For CelebA, we observe that, although the other three competitive methods can restore the facial contour, they do however lose a lot of detailed facial features. Thus, the denoised images of these methods are a blur with artifacts. In contrast, our denoising results are much clearer and closer to the ground truth images. For Flower and CUB-200 datasets, the foreground and background are more diverse and complicated than CelebA. Our results are clean with sharp edges (in close-up versions), while other methods have artifacts near and at the edges. This illustrates that \ourmodel can handle category-specific image denoising very well.

\begin{table*}[]
\centering
\caption{The performance comparison on the two remote sensing datasets.} %In the meantime, \ourmodel ($1.46\times10^6$) has fewer parameters as compared to Unet ($7.70\times10^6$).
% \resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline\hline
Dataset & $\sigma$ & EPLL~\cite{EPLL} & MemNet~\cite{Tai-MemNet-2017} & IRCNN~\cite{IRCNN} & REDNet~\cite{REDNet} & DnCNN~\cite{DnCNN} & FFDNet~\cite{zhang2018ffdnet} & \ourmodel \\ \hline
& 30 & 31.95 & 31.82 & 31.12 & 29.98 & 30.69 & 22.68 & \textbf{33.08} \\
& 50 & 29.65 & 27.71 & 27.50 & 28.82 & 26.99 & 24.17 & \textbf{31.14} \\
\multirow{-3}{*}{RICE1~\cite{RICE}} & 70 & 28.29 & 27.12 & 26.53 & 26.56 & 25.04 & 23.51 & \textbf{30.03} \\\hline
& 30 & 36.05 & \textbf{36.49} & 35.83 & 33.12 & 34.68 & 34.02 & 35.93 \\
& 50 & 33.22 & 33.62 & 33.74 & 30.40 & 29.57 & 30.26 & \textbf{34.71} \\
\multirow{-3}{*}{RICE2~\cite{RICE}} & 70 & 31.63 & 31.73 & 32.43 & 27.55 & 30.81 & 28.51 & \textbf{33.98} \\ \hline
\hline
\end{tabular}
% }
\label{Tab:RICE}
\end{table*}

\begin{figure}[t]
\centering
% remote sensing 1
\begin{subfigure}{.22\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/remote_sensing_2/contrast_RICE1_S0.001_corrupted_image_23.png}  
  \caption{Clean/Noisy}
  \label{fig:sub_clean/noisy}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
  \centering
  % I can't find the image for DnCNN. 
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/remote_sensing_2/contrast_RICE1_S0.001_DnCNN_denoised_image_23.png}  
  \caption{DnCNN}
  \label{fig:sub_DnCNN}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/remote_sensing_2/contrast_RICE1_S0.001_FFDNet_denoised_image_23.png}  
  \caption{FFDNet}
  \label{fig:sub_FFDNet}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/remote_sensing_2/contrast_RICE1_S0.001_glow_denoised_image_23.png}
  \caption{\ourmodel}
  \label{fig:sub_our}
\end{subfigure}

\caption{Visual results on RICE1 with Variance $=0.001$. For (a), the left part is the clean image and the right part is the noisy image. For~(b)-(d), the left part is the denoised image and the right region reflects the difference between the denoised and GT images. Whiter pixels represent better denoising performance. }
\label{fig:Visual_Rice}
\vspace{-6mm}
\end{figure}

\subsection{Remote Sensing Image Denoising}
\label{sec:Remote_Sensing}

\textbf{Quantitative Results.} 
The results of denoising the RICE datasets with $\sigma$ =30, 50, 70 AWGN are reported in Table~\ref{Tab:RICE}. \ourmodel improves by 1.13 dB-1.74 dB on RICE1 with different noise levels comparing with the highest results from other competitive methods. On RICE2, \ourmodel outperforms other methods when the noise levels are large, \ie achieving an increase of 0.97 dB and 1.55 dB for $\sigma$ =50 and 70, respectively. These results demonstrating that \ourmodel are also capable of restoring images following complex distributions. 

\textbf{Qualitative Results.} 
The visual results are shown in Figure~\ref{fig:Visual_Rice}\footnote{Although in RGB images, blacker pixels represent smaller values, we change every pixel in the right regions by using 255 minus the value, and thus whiter regions are smaller. }. The remote sensing datasets are mainly composed of images with two types of regions: the texture regions such as mountains, and the smooth regions, for example, deserts. An example of the smooth region from RICE1 with $\sigma=$ is taken. Our \ourmodel outperforms other methods significantly from the right regions of Figure~\ref{fig:sub_DnCNN}-\ref{fig:sub_our}.
Thus, our distribution learning and disentanglement based denoising method~\ourmodel has proven to be effective in denoising synthetic noise datasets, no matter whether the dataset is category-specific.

\subsection{Real Image Denoising} 
\begin{table*}
\centering
\caption{Comparisons on the real noisy SIDD dataset.When we train \ourmodel with SIDD medium dataset.} 
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\hline
\hline
Method & DnCNN~\cite{DnCNN} & TNRD~\cite{TNRD} & BM3D~\cite{BM3D} & WNNM~\cite{WNNM} & KSVD~\cite{KSVD} & CBDNet~\cite{Guo2019Cbdnet} & GradNet~\cite{liu2020gradnet} & AINDNet~\cite{AINDNet} & VDN~\cite{VDN} & \ourmodel\\ 
\hline
PSNR (dB) & 23.66 & 24.73 & 25.65 & 25.78 & 26.88 & 33.28 & 38.34 & 39.08 & 39.26 & 39.31 \\
SSIM & 0.583 & 0.643 & 0.685 & 0.809 & 0.842 & 0.868 & 0.953 & 0.946 & 0.955 & \\
Param (M) & 0.56 & -- & -- & -- & -- & 4.34 & 1.6 & 13.76 & 7.81 & 4.3 \\
\hline
\hline
\end{tabular}
}
\label{Tab:SIDD}
% \vspace{-4mm}
\end{table*}

\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{secs/images/Interpolation.pdf}
% \vspace{-3cm}
\caption{Using \ourmodel for noise data augmentation. The third row is the visual results of the generated noisy images corresponding to the clean images in the first row.}
\label{fig:Interpolation_SIDD}
% \vspace*{-6mm}
\end{figure}

\textbf{Quantitative Results.}
The performance comparison on the test set of the real noise dataset SIDD~\cite{SIDD_2018_CVPR} is listed in Table~\ref{Tab:SIDD}. 
We achieves competitive denoising accuracy comparing with other state-of-the-art methods. In addition, our model size (4.3M) is much smaller than the competitive AINDNet~\cite{AINDNet} (13.76M) and VDN~\cite{VDN} (7.81M).

\textbf{A Novel Data Augmentation Technique: }
The advantage of our distribution-learning based invertible denoising network is that we can generate new noisy image samples based on the learned distribution. This can decrease the workload on researchers for developing real noise datasets. To generate the new noisy dataset, we keep the clean latent variables the same during the decoding stage, while sampling from the noise distribution. To avoid outliers, we randomly interpolate between the latent variables for the clean images and those for the noisy images. A few generated noisy samples based on SIDD  are shown in Figure~\ref{fig:Interpolation_SIDD}. 


% For CelebA, our method improves by 1.26dB and 0.22dB for $\sigma=15$ and $50$, respectively, compared with the highest values by the other methods. We achieve similar improvements for Flower and CUB-200 as well.
%For CUB-200, we also improved 0.13dB - 0.47dB compared with Unet~\cite{Unet_2015}. %Furthermore, if we take the number of parameters of each network structure into consideration, 
% as shown in Table~\ref{Tab:parameter comparison}, 
%our \ourmodel only has one-fifth of the parameters of the Unet, demonstrating our model's superiority in noise removal. %Unet~\cite{Unet_2015}

%We report the PSNR and SSIM values of the denoised images for these 3 datasets in Table~\ref{Tab:Class_Specific AWGN Denoise}. Comparing with other competitive methods in synthetic noise removing, such as DnCNN, FFDNet and Unet, our Glow based method got the highest PSNR performance on almost all the datasets and noise levels. For CelebA, we increased 1.26dB and 0.73dB separately on $\sigma=15$ and $50$. For CUB-200, we also improved 0.13dB - 0.47dB compared with Unet. However, if we take the number of parameters of each network structure into consideration, as shown in Table~\ref{Tab:parameter comparison}, our Glow based denoising method only has one-fifth of the parameters of Unet, demonstrating our superiority in noise removing.


% % Here is the image. 
% \begin{comment}
% \begin{figure*}
% \centering
% \includegraphics[width=0.9\textwidth]{secs/images/Flower.pdf}
% % \vspace{-3cm}
% \caption{The comparisons on Flower for $\sigma=50$ against state-of-the-art method.}
% \label{fig:Visual_Flower}
% \end{figure*}
% \end{comment}

% \begin{comment}
% \begin{figure*}
% \centering
% \includegraphics[width=0.9\textwidth]{secs/images/Bird.pdf}
% % \vspace{-3cm}
% \caption{The visual comparison on CUB-200~\cite{??} for $\sigma=50$.}
% \label{fig:Visual_Bird}
% \end{figure*}
% \end{comment}

% \begin{table}\small
% \caption{The number of parameters for each network using CelebA.}
% \label{Tab:parameter comparison}
% \centering
% \begin{tabular}{l|c|c|c|c}
% \hline\hline
%  & DnCNN & FFDNet & GradNet & Glow \\ \hline
% Num & $1.48\times10^6$ & $0.85\times10^6$ & $1.29\times10^6$ & $1.46\times10^6$ \\
% \hline\hline
% \end{tabular}
% \vspace{-6mm}
% \end{table}

% \SA{Table caption should always be above and the Figure captions should be below.}

% \begin{table}\small
% \caption{The number of parameters for each network using CelebA. \SA{Table caption should always be above and the Figure captions should be below.}}
% \label{Tab:parameter comparison}
% \centering
% \begin{tabular}{l|c|c|c|c}
% \hline\hline
%  & DnCNN & FFDNet & Unet & Glow \\ \hline
% Num & $1.48\times10^6$ & $0.85\times10^6$ & $7.70\times10^6$ & $1.46\times10^6$ \\
% \hline\hline
% \end{tabular}
% \vspace{-6mm}
% \end{table}

% \begin{figure}
% \begin{centering}
% \includegraphics[width=0.48\textwidth]{secs/images/Denoise_Convergence.pdf}
% \caption{Convergence Speed Comparison.
% }
% \label{fig:Convergence}
% \end{centering}
% \end{figure}

%We also employ this structure for blind denoising with noise level between [0,55], as shown in Table~\ref{Tab:Class_Specific Blind Denoise}. The noise distribution of blind denoising is Gaussian Mixture Distribution, which is much more complicated than the Gaussian distribution with a certain noise level. Comparing with the structures with similiar number of parameters, i.e., DnCNN and FFDNet, our Glow based denoising model achieves an improvement of 2.13dB and 1.74dB separately on the CUB-200 dataset~\cite{Bird} and the Flower dataset~\cite{Flower}.

%The visual results are shown in Figure~\ref{fig:Visual_CelebA}, ~\ref{fig:Visual_Flower}, ~\ref{fig:Visual_Bird}. For CelebA, we can find that although the other three methods can restore the facial contour, they lost a lot of detailed facial features. Thus, the denoised images of these methods are blur with artifacts. On the contrary, the results of our Glow based denoising are much more clear and close to the ground truth images. For Flower and CUB-200, the foreground and background are more diverse and complicated than CelebA. When we zoom in, we can see our results are clean with sharp edges while other methods got artifacts in the edges. This illustrates Glow based denoising method can handle specific category image denoising very well.
% invertiblity keeps information; category specific images has fixed patterns;

% \begin{table}\small
% \centering
% \caption{Blind denoising quantitative results on three category-specific datasets. The noise follows a Gaussian Mixture Distribution, and the level is between $[0, 55]$.}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lcccccccc}
% \hline
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{DnCNN} & \multicolumn{2}{c}{FFDNet} & \multicolumn{2}{c}{\ourmodel} \\ 
% \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
% CelebA  & 30.34 & 0.95 & 30.84 & 0.95 & \textbf{30.85} & \textbf{0.96} \\ \hline
% CUB-200 & 28.71 & 0.92 & 28.46 & 0.92 & \textbf{30.59} & \textbf{0.94} \\ \hline
% Flower  & 28.40 & 0.94 & 28.69 & 0.95 & \textbf{30.43} & \textbf{0.96} \\ \hline
% \end{tabular}
% }
% \label{Tab:Class_Specific Blind Denoise}
% % \vspace{-6mm}
% \end{table}

% \begin{table}\small
% \centering
% \caption{Blind denoising quantitative results on three category-specific datasets. The noise follows a Gaussian Mixture Distribution, and the level is between $[0, 55]$.}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lcccccccc}
% \hline
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{DnCNN} & \multicolumn{2}{c}{FFDNet} & \multicolumn{2}{c}{GradNet} & \multicolumn{2}{c}{Glow} \\ 
% \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
% CelebA  & 30.34 & 0.95 & 30.84 & 0.95 & & & \textbf{30.85} & \textbf{0.96} \\ \hline
% CUB-200 & 28.71 & 0.92 & 28.46 & 0.92 & \textbf{30.86} & 0.94 & \textbf{30.59} & \textbf{0.94} \\ \hline
% Flower  & 28.40 & 0.94 & 28.69 & 0.95 & 28.84 & 0.94 & \textbf{30.43} & \textbf{0.96} \\ \hline
% \end{tabular}
% }
% \label{Tab:Class_Specific Blind Denoise}
% \vspace{-6mm}
% \end{table}

% \textbf{Comparisons of parameters and convergence speed.}
% We use a 40 layer DnCNN. The comparison of number of parameters is listed in Table~\ref{Tab:Face Denoising Performance Comparision}. Our structure achieves higher denoising accuracy with less parameters compared with DnCNN.

% \begin{table*}[]
% \centering
% \caption{The performance comparison on the two remote sensing datasets.}
% \begin{tabular}{llcccccccccc}
% \hline
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{DnCNN} & \multicolumn{2}{c}{FFDNet} &
% \multicolumn{2}{c}{Unet} &
% \multicolumn{2}{c}{GradNet} & \multicolumn{2}{c}{Glow}  \\ 
% \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{-2}{*}{Variance}} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
% & 0.001 & 36.53 & 0.9832 & 36.85 & 0.9749 & 39.40 & 0.9901 & 39.32 & \textbf{0.9894} & \textbf{39.92} &  0.9874 \\
% & 0.005 & 33.86 & 0.9678 & 35.04 & 0.9696 & 36.47 & \textbf{0.9799} & 35.42 & 0.9750 & \textbf{36.56} &  0.9755 \\
% \multirow{-3}{*}{RICE1} & 0.01 & 33.34 & 0.9612 & 33.99 & 0.9642 & 35.12 & \textbf{0.9739} & 34.01 & 0.9674 & \textbf{35.17} & 0.9685 \\ \hline
% & 0.001 & 41.34 & 0.9928 & 42.40 & 0.9931 & 44.01 & \textbf{0.9957} & 44.01 & 0.9956 & \textbf{44.66} & 0.9954 \\
% & 0.005 & 39.19 & 0.9887 & 39.97 & 0.9896 & \textbf{42.30} & \textbf{0.9929} & 39.54 & 0.9891 & 41.70 & 0.9915 \\ 
% \multirow{-3}{*}{RICE2} & 0.01 & 37.76 & 0.9831 & 39.23 & 0.9884 & 40.28 & 0.9899 & \textbf{40.59} & \textbf{0.9905} & 40.30 & 0.9890\\ \hline
% \end{tabular}
% \label{Tab:RICE}
% \end{table*}

% \begin{table*}[]
% \centering
% \caption{The performance comparison on the two remote sensing datasets.}
% \begin{tabular}{llcccccccc}
% \hline
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{DnCNN} & \multicolumn{2}{c}{FFDNet} & \multicolumn{2}{c}{GradNet} & \multicolumn{2}{c}{\ourmodel}  \\
% \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{-2}{*}{Variance}} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
% & 0.001 & 36.53 & 0.9832 & 36.85 & 0.9749 & 39.32 & \textbf{0.9894} & \textbf{39.92} &  0.9874 \\
% & 0.005 & 33.86 & 0.9678 & 35.04 & 0.9696 & 35.42 & 0.9750 & \textbf{36.56} &  \textbf{0.9755} \\
% \multirow{-3}{*}{RICE1} & 0.01 & 33.34 & 0.9612 & 33.99 & 0.9642 & 34.01 & 0.9674 & \textbf{35.17} & \textbf{0.9685} \\ \hline
% & 0.001 & 41.34 & 0.9928 & 42.40 & 0.9931 & 44.01 & \textbf{0.9956} & \textbf{44.66} & 0.9954 \\
% & 0.005 & 39.19 & 0.9887 & 39.97 & 0.9896 & 39.54 & 0.9891 & \textbf{41.70} & \textbf{0.9915} \\ 
% \multirow{-3}{*}{RICE2} & 0.01 & 37.76 & 0.9831 & 39.23 & 0.9884 & \textbf{40.59} & \textbf{0.9905} & 40.30 & 0.9890\\ \hline
% \end{tabular}
% \label{Tab:RICE}
% \vspace{-2mm}
% \end{table*}

% \begin{table*}[]
% \centering
% \caption{The performance comparison on the two remote sensing datasets..}
% \begin{tabular}{llcccccccc}
% \hline
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{DnCNN} & \multicolumn{2}{c}{FFDNet} & \multicolumn{2}{c}{Unet} & \multicolumn{2}{c}{Glow}  \\ 
% \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{-2}{*}{Variance}} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
% & 0.001 & 36.53 & 0.9832 & 36.85 & 0.9749 & 39.40 & 0.9901 & \textbf{39.92} &  0.9874 \\
% & 0.005 & 33.86 & 0.9678 & 35.04 & 0.9696 & 36.47 & 0.9799 & \textbf{36.56} &  0.9755 \\
% \multirow{-3}{*}{RICE1} & 0.01 & 33.34 & 0.9612 & 33.99 & 0.9642 & 35.12 & 0.9739 & \textbf{35.17} & 0.9685 \\ \hline
% & 0.001 & 41.34 & 0.9928 & 42.40 & 0.9931 & 44.01 & 0.9957 & \textbf{44.66} & 0.9954 \\
% & 0.005 & 39.19 & 0.9887 & 39.97 & 0.9896 & \textbf{42.30} & 0.9929 & 41.70 & 0.9915 \\ 
% \multirow{-3}{*}{RICE2} & 0.01 & 37.76 & 0.9831 & 39.23 & 0.9884 & 40.28 & 0.9899 & \textbf{40.30} & 0.9890\\ \hline
% \end{tabular}
% \label{Tab:RICE}
% \end{table*}

% remote sensing 2
% \begin{subfigure}{.22\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=.99\linewidth]{secs/images/remote_sensing_1/contrast_RICE2_S0.001_corrupted_image_11.png}  
%   \caption{Clean/Noisy}
% \end{subfigure}
% \begin{subfigure}{.22\textwidth}
%   \centering
%   % I can't find the image for DnCNN. 
%   % include second image
%   \includegraphics[width=.99\linewidth]{secs/images/remote_sensing_1/contrast_RICE1_S0.001_DnCNN_denoised_image_11.png}  
%   \caption{DnCNN}
% \end{subfigure}
% \begin{subfigure}{.22\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=.99\linewidth]{secs/images/remote_sensing_1/contrast_RICE1_S0.001_FFDNet_denoised_image_11.png}  
%   \caption{FFDNet}
% \end{subfigure}
% \begin{subfigure}{.22\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=.99\linewidth]{secs/images/remote_sensing_1/contrast_RICE1_S0.001_glow_denoised_image_11.png}
%   \caption{\ourmodel}
% \end{subfigure}

% One of the most important applications of image denoising is the denoising of remote sensing images for further processing. Since the remote sensing datasets contain diverse terrains and features in different images, the distribution of remote sensing dataset is much more complicated than category specific images like face. So we also tried our method on 2 remote sensing datasets to see the effectiveness when the distribution of the ground truth images become complex.

% \textbf{Datasets.}
% \textbf{Training Details.} 

% , and achieves similar or better accuracy with Unet when the noise level becomes larger. Meanwhile, we have much fewer parameters than Unet.

% \begin{comment}
% \begin{figure*}
% \centering
% \includegraphics[width=0.9\textwidth]{secs/images/RICE1.pdf}
% % \vspace{-3cm}
% \caption{Visual results on RICE1 with Variance of $=0.001$. There are texture regions and smooth regions in this dataset. Taking a sample from each of the two regions, and the results are illustrated above. Please zoom in for details.}
% \label{fig:Visual_RICE}
% \end{figure*}
% \end{comment}

% We take two samples from RICE1~\cite{RICE} for each of the two regions. For the texture region in the first row, our method achieves almost the same visual results as Unet. However, the PSNR value is higher than the denoised image from DnCNN, FFDNet, and Unet. It is a little bit difficult to perceive the difference visually. However, our \ourmodel's superiority is evident in the second row's smooth region. When we zoom in this region, some dark rectangle regions can be observed in the ground truth image. DnCNN~\cite{DnCNN} removes all the dark regions, and Unet~\cite{Unet_2015} generates new artifacts. Our method may seem to have achieved visually  similar results as FFDNet~\cite{zhang2018ffdnet}, but we have an improvement of 1.68dB based on PSNR. This considerable improvement will benefit the follow-up processing for remote sensing data analyses. 

%The visual results are shown in Figure~\ref{fig:Visual_RICE}. The remote sensing dataset contains images for two kinds of regions, the texture regions like mountains and the smooth regions like  deserts. We take two samples from RICE1 from each of the two regions. For the texture region in the first row, the glow base denoising method achieves almost the same visual results as Unet. Although the PSNR value is higher than the denoised image by DnCNN, FFDNet and Unet, it's a little bit hard to tell the difference visually. However, the superiority of Glow based denoising method is much clear in smooth region in the second row. When we zoom in this region, some dark rectangle regions can be found in the ground truth image. DnCNN removes all the dark regions and Unet leaves artifacts. Glow based denoising method achieves similar visual results as FFDNet but has an improvement of 1.68dB based on PSNR. This large margin improvement will benefit the follow-up processing for remote sensing data analyses. 

% \textbf{Why Remote Sensing Dataset?}
% \SA{The title should be: Why remote sensing dataset? or the need for remote-sensing dataset}
% One may argue that the experiment on category-specific and remote sensing images both employ synthetic noisy datasets, so there is no need to verify the capacity of \ourmodel again. However, category-specific images usually have similar patterns in all the images. Taking the face dataset as an example, the facial contours and facial features of different people follow the same distribution, although each person's details might be different. Since we aim to disentangle the distributions of the ground truth clean images from the noise, it is easier for our method to learn on data that obviously follows the same distribution. On the contrary, the patterns in remote sensing datasets are different and much more complicated, including mountains, deserts, forests, \etc Some of the regions are full of textures, but some are smooth. These experiments verify that even in these complex situations, our method can also achieve mostly better denoising accuracy than the competitive feature-learning based methods. This demonstrates the feasibility and potential of our newly designed distribution-learning based method for image denoising.

%Someone may argue that the experiment on remote sensing datasets and category-specific datasets are both synthetic AWGN removing, so there is no need to verify the capacity of Glow based denoising again. However, category-specific images usually have similar patterns in all the images. Taking the face dataset as an example, the facial contours and facial features of different people follows the same distribution, although the details for each person might be different. Since we aim at disentangling the distribution of the ground truth clean image from the noisy image, it is easier for our method to learn on data which obviously follows the same distribution. On the contrary, the patterns in remote sensing datasets are different and much more complicated, including the mountains, deserts, forests etc. Some of the regions are full of textures but some are smooth. This group of experiment verifies that even in this complex situation, the Glow based method can also achieves similar or better denoising accuracy than other competitive feature-learning based method. This demonstrates the feasibility and potential of designing new distribution-learning based method for image denoising.

% \SA{Better title would be Real Image Denoising}
% After trying on the complex ground truth images which follow complicated distributions, we also want to verify the capacity of our method in removing complicated real noise instead of limiting in the simpler synthetic noise. We conduct real noise removing on the real noise dataset SIDD~\cite{SIDD_2018_CVPR}. \textbf{SIDD}~\cite{SIDD_2018_CVPR} is taken by five smartphone cameras with small apertures and sensor sizes. The small SIDD dataset contains 160 noisy and noise-free pairs and the medium SIDD dataset have 320 pairs. They are cropped into $256\times256$ patches during training.

% The authors provide 200 noisy and noise-free pairs, where 160 image pairs can be used for training, and the remaining 40 pairs as validation. The test set is composed of another 1280 noisy images without the corresponding noise-free patches.
% The training set is randomly cropped from three real noise datasets, \ie SIDD~\cite{SIDD_2018_CVPR}, PolyU~\cite{PolyU} and Renoir~\cite{anaya2014renoir}, resulting in 2000 $512\times512$ patch pairs for training. This strategy of generating training set follows RIDNet~\cite{RIDNet}, CBDNet~\cite{Guo2019Cbdnet} and FFDNet~\cite{zhang2018ffdnet}, which not only increase the diversity of noise and texture distributions exposed to the network but also keep the training size not too large to save the training time. 
% These patches are randomly cropped into $80\times80$ patches during training. 

% \begin{table}
% \centering
% \caption{Comparisons on the real noisy SIDD dataset.When we train \ourmodel with SIDD medium dataset, we achieve better SSIM than other methods.}
% \begin{tabular}{l|c|c}
% \hline
% \multirow{2}{2em}{Method} & \multicolumn{2}{c}{SIDD}\\
% \cline{2-3}
%  & PSNR & SSIM \\
% \hline
% DnCNN~\cite{DnCNN}  & 23.66 & 0.583 \\ \hline
% TNRD~\cite{TNRD}  & 24.73 & 0.643 \\ \hline
% BM3D~\cite{BM3D}  & 25.65 & 0.685 \\ \hline
% WNNM & 25.78 & 0.809 \\ \hline
% KSVD~\cite{KSVD} & 26.88 & 0.842 \\ \hline
% EPLL & 27.11 & 0.870 \\ \hline
% CBDNet~\cite{Guo2019Cbdnet} & 33.28 & 0.868 \\ \hline
% NCSR & 34.05 & 0.8351 \\ \hline
% DeepProxies BM3D & 34.34 & 0.911 \\ \hline
% GradNet~\cite{Liu_2018_CVPR_Workshops} & 38.34 & 0.946 \\ \hline
% VDN~\cite{VDN} & 39.26 & 0.955 \\ \hline
% CycleISP~\cite{CycleISP} & 39.52 & 0.957 \\ \hline
% \ourmodel & 39.31 & \\ \hline
% % \ourmodel (small) & 34.42 & 0.9531 \\ \hline
% % Glow (small + aug) & 34.38 & 0.9527 \\ \hline
% % \ourmodel (medium) & 36.46 & 0.9703 \\ \hline
% \end{tabular}
% \vspace{-2mm}
% %  \SA{our SSIM is better than all methods}
% % The mean PSNR and SSIM are reported.%denoising results of algorithms evaluated on the DnD sRGB and SIDD sRGB datasets}
% \label{Tab:SIDD}
% \vspace*{-2mm}
% \end{table}

% We trained with the small SIDD dataset first and got an accuracy of 34.42dB. Although our result cannot outperform the state-of-the-art on this dataset in terms of PSNR, we have achieved comparative results on SSIM. Furthermore, we value its denoising capacity and potential as the first attempt to disentangle the ground truth and noise distributions. 

%The comparison of our Glow based denoising method with other methods are listed in Table~\ref{Tab:SIDD}. We tried training with the small SIDD dataset first and got an accuracy 34.42dB. Although this result cannot beat the state-of-the-art on this dataset, as the first attempt to disentangle the ground truth and noise distributions, we value its denoising capacity and potential. 

% \textbf{Real Denoising Limitations.}
% The reason for this not so competitive result in terms of PSNR might be twofold: 1) the distribution of noise is complicated, and 2) the distribution of ground truth images is difficult to learn. 

% For the first reason, since the noise distribution is complicated, it will be better to use as large a sample as possible to capture this distribution during training. However, this small dataset only has 160 image pairs, which is very limited to learn complicated real noise distribution. To verify this, we train a model with the medium dataset, containing 320 image pairs. This dataset has almost the same ground truth clean images for the same scenes as the small dataset but has more noisy images. With this dataset, we achieved the PSNR of \textbf{36.46dB}, more than \textbf{2dB} higher compared to the small one; moreover, we are the best in terms of SSIM. This improvement illustrates that our denoising method requires large real noisy samples to learn a better distribution.

% For the second reason, similar to Section~\ref{sec:Remote_Sensing} remote sensing dataset, the distribution of the ground truth scenes of SIDD is also complicated. A possible technique to avoid the complicated clean image problem might lie in disentangling the high-frequency of the noisy images instead of disentangling the ground truth and noise. The distribution of noise is a part of the high-frequency distribution. We would explore this direction in our future work.


%The reason of this not so competitive result might lie in twofold: one is that the distribution of noise is complicated and the other is that the distribution of ground truth images is hard to learn. 
%For the first reason, since the noise distribution is complicated, it will be better to use as much sample as possible from this distribution for training. However, this small dataset only has 160 image pairs, which is very limited to learn the complicated real noise distribution. To verify this, we also train a model with the medium dataset, containing 320 image pairs. This dataset has almost the same ground truth clean images for the same scenes with the small dataset but have different noise images. With this dataset, we got the PSNR result 36.46dB, 2dB higher than the small one. The improvement illustrates that Glow based denoising method need large real noise samples to learn the distribution better.
%For the second reason, similar to what we have stated in Section~\ref{sec:Remote_Sensing} for remote sensing dataset, the distribution of the ground truth scenes of SIDD is also complicated. A potential way to avoid the complicated clean image problem might lie in disentangling the high frequency of the noisy images instead of disentangling the ground truth and noise. The distribution of noise is a part of the high frequency distribution. We leave this guess as our future work to verify.

% \st{However, when we train the model with a small SIDD dataset, and this data augmentation method, we got 34.38 dB, which is almost the same as training without data augmentation. We guess there are some defects for disentangling two distributions directly, which might mislead the generated noisy images. Since we are the first to explore the disentanglement of two distributions, we will leave this problem for future work to explore.}

%The advantage of our distribution based invertible denoising network is that we can generate new noisy image samples based on the distribution we learnt. This can reduce the workload of taking real noise datasets. The way to do this is that, during the decode stage, we keep the clean latent variables the same while randomly sample from the noise distribution. To avoid the outliers, we randomly interpolate between the latent variables for the clean images and those for the noisy images. Some samples of the generated noisy images are illustrated in Figure~\ref{fig:Interpolation_SIDD}. 

%However, when we train the model with small SIDD dataset and this data augmentation method, the result we got is 34.38 dB, which is almost the same as training without data augmentation. We guess there are some defects for disentangling two distributions directly, which might mislead the generated noisy images. Since we are the first to explore the disentanglement of two distributions, we will leave this problem for future work to explore.

% \begin{table*}[t]\small                                                      
% \caption{Real image denoising on SIDD.}
% \label{Tab:Blind Denoising}
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% \hline\hline
% Methods & DnCNN & BM3D~\cite{BM3D} & WNNM & KSVD &  CBDNet~\cite{Guo2019Cbdnet} & AINDNet~\cite{AINDNet} & VDN~\cite{VDN} & CycleISP~\cite{CycleISP} & Glow \\ \hline
% PSNR & 30.71 & 25.65 & 25.78 & 26.88 & 33.28 & 39.08 & 39.26 & 39.52 & 36.46 \\ \hline
% SSIM & 0.695 & 0.685 & 0.809 & 0.842 & 0.868 & 0.953 & 0.955 & 0.957 & 0.9703 \\ \hline
% \hline
% \end{tabular}
% % \vspace{-2mm}
% % \vspace{-1.2em}
% \end{table*}

% \begin{table*}\small                                                      
% \caption{Real image denoising on DND.}
% \label{Tab:Blind Denoising}
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|c}
% \hline\hline
% Methods & CIMM~\cite{CIMM} & RIDNet~\cite{RIDNet} & AINDNet~\cite{AINDNet} & VDN~\cite{VDN} & CycleISP~\cite{CycleISP} & GAE (w/o T) & GAE (T) \\ \hline
% PSNR & 39.20 & 39.26 & 39.7695 & 39.383 & 39.56 & &  \\ \hline
% SSIM & 0.9524 & 0.9528 & 0.959 & 0.9518 & 0.9564 & & \\ \hline
% \hline
% \end{tabular}
% % \vspace{-2mm}
% % \vspace{-1.2em}
% \end{table*}



% \begin{table}
% \centering
% \caption{Comparisons on the denoising accuracy of different numbers of DownScale Blocks and Invertible Blocks.} 
% \begin{tabular}{cccc}
% \hline
% \hline
% Flow Blocks & SoF Blocks & PSNR \\ 
% \hline
% 1 & 8 & 38.00   \\ 
% 2 & 8 & \textbf{\textcolor{red}{38.40}}   \\ 
% 3 & 8 & 37.69   \\ \hline
% 1 & 16 & 38.30   \\ 
% 2 & 16 & \textbf{\textcolor{red}{38.61}}   \\ 
% 3 & 16 & 38.15   \\ \hline
% \hline
% \end{tabular}
% \label{Tab:Scale}
% \vspace{-4mm}
% \end{table}




==> secs/Intro_old.tex <==
\section{Introduction}
% Importance of image denoising
Despite decades of research, image denoising~\cite{RIDNet}~\cite{liu2020gradnet} is still an on-going low-level image processing task in computer vision. The long-standing interest in image denoising has provided roots for a vast array of downstream applications, such as segmentation~\cite{minaee2020image} or deblurring~\cite{Zhang_2017_CVPR}. Nearly all images require to be denoised before further processing, especially those obtained in dark environments. Recently, neural networks based image denoising methods~\cite{DnCNN}~\cite{zhang2018ffdnet}~\cite{VDN} have made substantial improvements over traditional approaches~\cite{BM3D}~\cite{2017_TV_wavelet_non_local}. 

\begin{figure}[ht]
\centering
\begin{subfigure}{.14\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_5/box_bird_gt_image_70.png}  
  \caption*{GT}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.14\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_5/cropped_bird_S50.0_corrupted_image_70.png}  
  \caption*{Noisy}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}{.14\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_5/cropped_bird_S50.0_DnCNN_denoised_image_70.png}  
  \caption*{DnCNN: 28.43dB}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}{.14\textwidth}
  \centering
  % include first image
  \includegraphics[width=.99\linewidth]{secs/images/bird_5/cropped_bird_S50.0_FFDNet_denoised_image_70.png}  
  \caption*{FFDNet: 27.77dB}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.14\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_5/cropped_bird_S50.0_dncnn_sk_conGradient_before_denoised_image_70.png}  
  \caption*{GradNet: 29.47dB}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}{.14\textwidth}
  \centering
  % include second image
  \includegraphics[width=.99\linewidth]{secs/images/bird_5/cropped_bird_S50.0_glow_denoised_image_70.png}  
  \caption*{\ourmodel: 30.00dB}
  \label{fig:sub-second}
\end{subfigure}
\caption{The comparison of denoising results on CUB-200 with $\sigma=50$ AWGN (Additive White Gaussian Noise).}
\label{fig:Visual_Bird}
\end{figure}

% Brief introduction of image denoising task
Image denoising is to reconstruct clean images from corrupted noisy observations.
Traditional denoising methods employ assumptions on noise distribution~\cite{6751276}~\cite{7557070} or priors on ground truth clean images~\cite{BM3D}~\cite{6122031} to build optimization models. However, these assumptions and priors might be different from the real case, resulting in compromising the denoising accuracy.
Deep learning denoising approaches proposed in recent years using convolutional neural networks (CNNs) to learn the models from a large amount of noise-free and noisy image pairs and have achieved superior denoising accuracy~\cite{DnCNN}~\cite{zhang2018ffdnet}.
These networks employ CNNs to extract discriminative feature maps and learn the mapping functions between noisy images and clean ones or noise. However, these methods usually overemphasize the pixel similarity between the denoised image and the clean ground truth while omit the underlying distribution of the clean images. Thus, although some deep methods can obtain high quantitative results, over-smoothed regions and artifacts are usually brought into the restored images, resulting in degraded visual results.
 
% why we use invertible glow like structure
This paper rethinks image denoising from the distribution perspective.
The distribution of noisy images can be treated as a joint distribution of clean images and noise. Thus, it is intuitive to consider conducting image denoising via disentangling these two distributions. 
Following this line of thought, the distribution-learning based image denoising can be divided into three stages: the first is to learn the distribution of noisy images, the second is to disentangle the distribution of clean images from the noisy ones, and the last is to generate clean images from the disentangled clean representation. 

There are two challenges for us to overcome: which kind of network is suitable for learning the distributions and restoring images; how to disentangle the two distributions.
For the first problem, we resort to generative models to learn the distributions. We require the generative model can generate the denoised image given the disentangled latent code. The denoised image should not only follows a clean image distribution but also be visually similar to the corresponding noisy image. Therefore, the candidate generative model should has one-to-one mapping between the noisy image space and the latent space. Besides, a subspace of the latent space, i.e., the space of the disentangled latent code for clean images, can also be one-to-one mapped to the clean image space. However, variational autoencoder (VAE)~\cite{VAE} cannot guarantee the one-to-one mapping between the latent representations and images. On the other hand, although generative adversarial network (GAN) can insure the one-to-one mapping~\cite{ma2018invertibility}, learning two different distributions, i.e., the distributions of noisy and clean images, requires two discriminative networks, making the design not so elegant. 
Hence, we adopt normalizing flow~\cite{RealNVP}~\cite{Glow}, an invertible generative model, to learn the distributions and design the denoising algorithm.

The advantages of normalizing flow are reflected in three aspects. First, its invertibility ensures one-to-one mapping between images and their latent representations~\cite{liu2020deep}. This makes it possible to generate denoised images which are visually similar to the noisy images if we can disentangle the latent code of the clean ground truth from the latent representations appropriately. Second, it is capable of transforming complex distributions to independent distributions without losing information~\cite{liu2020deep}. Thus, we can obtain the accurate noisy distributions and also restore the clean images more accurately. Last, it parallelizes the training of encoder and decoder, making the model size much smaller and the training more efficient.

For the second challenge, we take advantage of the characteristics of the latent variables, which follows a distribution of $N(\bm{0}, \bm{I})$, that the dimensions are independent of each other. We assume that these dimensions can be disentangled into two groups, i.e., some of the dimensions encode clean images while the others encode noise. If we set the noise dimensions to constants, such as $\bm{0}$, the joint distribution of the clean dimensions and new noise dimensions will be the same as the marginal distribution of the clean images. The denoised images can be obtained through passing the new latent representations to the reverse of the network.

The contributions of this work are listed below.
\begin{itemize}
    \item We rethink the image denoising task and present a distribution-learning based denoising framework, which especially suits for category-specific image denoising.
    \item We propose a Flow-Based Image Denoising Neural Network (FDN). Different from the widely used feature-learning based CNNs in this area, \ourmodel learns the distribution of noisy images instead of low-level features.
    \item We present a disentanglement method to obtain the distribution of clean ground truth from the noisy distribution, without making any assumptions on noise or employing the priors of images.
    \item We achieve competitive performance in removing synthetic noise from category-specific images and remote sensing images. For real noise, we also verify the denoising capacity and potential of our architecture.
    \item \ourmodel can also be employed for data augmentation, i.e., generating noisy images by sampling new noisy latent representations, without any extra information needed.
\end{itemize}

% is that we provide a new perspective from which to understand the image denoising task, as well as a Flow-Based Image Denoising Neural Network (\ourmodel). Different from the widely used feature-learning based CNN networks in this area, we propose to disentangle the two distributions of the clean images and noises for denoising, without making assumptions of neither images nor noises. 
% This architecture achieves competitive performance in removing synthetic noise from category-specific images and remote sensing images. For real noise, we also verify the denoising capacity and potential of our architecture, and discuss the limitations. In addition, our method can be employed as a new method of data augmentation for generating noisy images using real noisy latent representation sampling.

% We aim to understand the denoising task from a different perspective from the previous feature-learning based discriminative models.

% Normalizing flows are invertible and their invertibility ensures one-to-one mapping between images and their latent representations.
% In addition, they are capable of transforming complex distributions to independent distributions without losing information~\cite{liu2020deep}. Thus, we explore their potential in denoising.
% The advantages of normalizing flows are threefold. First, compared to VAEs~\cite{VAE}, it is tractable to get the exact log-likelihood of very complex distributions and make exact latent-variable inferences via normalizing flows. Second, normalizing flows parallelize the training of encoder and decoder, which makes the model size much smaller than auto-encoders, \eg, Unet~\cite{Unet_2015}. Last, their invertibility allows us to get back to the original image space after manipulating the latent variables in the latent space. This makes it possible to generate denoised images with pixel match if we can disentangle the latent representation of noise from the noisy images appropriately.

% To learn complex distributions, it is natural to resort to generative models, since they are designed to inference distributions of the give data. 
% Generative models are considered here due to their capacity of learning complex distributions. 
% However, it is problematic if we apply generative models to generate the denoised images directly. To view image denoising as a generative process, we require the generative models for image denoising to map an image to a single latent representation in a one-to-one fashion. However, the one-to-one requirement is not aligned with the common requirements for building generative models. Standard generative models do not demand the one-to-one mapping between the input and the latent representation. For example, judged from citations, the two mainstream generative models are variational autoencoders (VAEs)~\cite{VAE} and generative adversarial networks (GANs)~\cite{goodfellow2014generative}; neither VAEs nor GANs map an input image to a unique latent representation. As a result, a generated denoised image may be quite different visually from its clean ground truth and this process should not properly be considered as denoising. Thus, to solve this problem, we resort to more recently proposed generative models that are gaining increasing attention: the flow-based generative models, \ie, normalizing flows~\cite{kobyzev2020normalizing}. 

% Normalizing flows are invertible and their invertibility ensures one-to-one mapping between images and their latent representations.
% In addition, they are capable of transforming complex distributions to independent distributions without losing information~\cite{liu2020deep}. Thus, we explore their potential in denoising.
% The advantages of normalizing flows are threefold. First, compared to VAEs~\cite{VAE}, it is tractable to get the exact log-likelihood of very complex distributions and make exact latent-variable inferences via normalizing flows. Second, normalizing flows parallelize the training of encoder and decoder, which makes the model size much smaller than auto-encoders, \eg, Unet~\cite{Unet_2015}. Last, their invertibility allows us to get back to the original image space after manipulating the latent variables in the latent space. This makes it possible to generate denoised images with pixel match if we can disentangle the latent representation of noise from the noisy images appropriately.
% % ZQ: Do we really need to say a lot of advantages of normalizing flows in the introduction? 

% This paper utilizes normalizing flow architectures to learn the latent representations of the noisy images, followed by disentangling the latent variables of the clean distribution and the noise distribution. The denoised images are obtained through reversing the clean latent representations to the original image space. 

% our contribution
% The main contribution of this work is that we provide a new perspective from which to understand the image denoising task, as well as a Flow-Based Image Denoising Neural Network (\ourmodel). Different from the widely used feature-learning based CNN networks in this area, we propose to disentangle the two distributions of the clean images and noises for denoising, without making assumptions of neither images nor noises. 
% This architecture achieves competitive performance in removing synthetic noise from category-specific images and remote sensing images. For real noise, we also verify the denoising capacity and potential of our architecture, and discuss the limitations. In addition, our method can be employed as a new method of data augmentation for generating noisy images using real noisy latent representation sampling.

==> secs/Methods_old.tex <==
\section{Methods}
In this section, we explain the design concept of \ourmodel first. Then we introduce the detailed components of the network architecture. The objective function as well as some training details are also presented. 

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{../secs/images/Concept.pdf}
\caption{The framework of distribution learning and disentanglement based image denoising.}   
\label{fig:framework}
% \vspace{-5mm}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{secs/images/Archi.pdf}
% \vspace{-3cm}
\caption{Network architecture of \ourmodel. \ourmodel consists of several invertible DownScale Flow Blocks. The forward pass encodes the corrupted image to latent variables $\bm{z} = (\bm{z_N}, \bm{z_C}) \sim \ngaussian$. The latent representations of noise $\bm{z_N}$ are set to $\bm{0}$, combined with the clean latent variables $\bm{z_C}$ as a new latent representation $\hatz$. The backward pass decodes $\hatz$ to the denoised image.}
\label{fig:NetArchi}
\end{figure*}


\subsection{Concept of Design}
We rethink the image denoising task from the perspective of distribution learning and disentanglement. 
Suppose the noisy image is $\y$ and the corresponding clean ground truth is $\x$. The noise $\n = \y-\x $. 
We have: $p(\y) = p(\x, \n) =  p(\x) p(\n | \x)$. That is, the distribution of the noisy images $p(\y)$ is a joint distribution of clean images and noise. In addition, the clean representation can be achieved if we can disentangle the clean and noise representations from $p(\y)$. Then, the clean images can be restored with the disentangled clean representation.

A framework of this scheme is presented in~\autoref{fig:framework}.
Our framework contains three steps, \textbf{first}, learn the distribution of noisy images by encoding $\y$ to a noisy latent representation $\z$; \textbf{second}, disentangle the clean representation $\zc$ from $\z$;
\textbf{last}, restore the clean image by decoding $\zc$ to the clean image space.
To ensure the denoising effect, the mappings between $\y$ and $\z$, $\zc$ and $\x$ should be one-to-one.

% Suppose the noisy image is $\y$ and the corresponding clean ground truth is $\x$. The noise $\n$ is $(\y-\x)$. 
% We have: $p(\y) = p(\x, \n) =  p(\x) p(\n | \x)$.
An invertible normalizing flow based network is employed to learn the distribution of noisy images $p(\y)$, transforming $\y$ to latent variables $\z$ following an simple prior distribution $\ngaussian$. Thus,

\begin{equation}
    p(\y) = p(\x) p(\n | \x) =p(\z)\big|\det(\frac{\partial f(\z)}{\partial \z})|\big|^{-1}, 
\end{equation}
where $f(\cdot)$ is the model learned by the network. The dimensions of $\z$ are independent of each other.

We assume $\z$ can be disentangled and some of the dimensions of $\z$ encode the distribution of clean images (denoted as $\zc$) and the remaining embeds noise (denoted as $\zn$). The clean image $\x$ can be restored through the following transformation:
\begin{equation}
    p(\x) =p(\zc)\big|\det(\frac{\partial f(\z)}{\partial \zc})\big|^{-1}. 
\label{Equ:p_x}
\end{equation}

However, how to obtain $\zc$ with $\z$ is not so obvious.
We propose a way of disentanglement by setting $\zn=\bm{0}$, that is,  
\begin{equation}
    \hatz = A\z, 
\end{equation}
where $A$ is a mask where is 1 in the dimensions for clean variables and 0 in those for noise. $\hatz$ is a new latent code which only contains the clean representations.
Thus, we have $p({\zn=\bm{0}})=1$ and the distribution of $\hatz$ becomes

\begin{equation}
    p(\hatz) =p(\zc)p(\zn)=p(\zc).
\end{equation}
Then the clean image can be obtained via \autoref{Equ:p_x}.

\subsection{Network Architecture}
The details of our \ourmodel architecture is introduced in this section. \ourmodel is composed of several invertible DownScale Flow Blocks, as presented in~\autoref{fig:NetArchi}. Each block consists of a Squeeze layer to downscale the latent representations followed by several Step-Of-Flow Blocks to perform distribution transformation. The details of each layer is presented as below.

\textbf{Squeeze.} The Squeeze layers take every other element of the intermediate latent variables, resulting in new downscaled latent representations with quadruple channels, as shown in \autoref{fig:Transform}.

\begin{figure}
\centering
\includegraphics[width=0.48\textwidth]{../secs/images/Squeeze.pdf}
\caption{The Squeeze operation downscales latent representations according to a checkerboard pattern.}   
\label{fig:Transform}
\vspace{-5mm}
\end{figure}

\textbf{Actnorm.} The Actnorm layers apply affine transformation on latent variables, as illustrated in Eq.~\eqref{Equ: Actnorm}. 
\begin{equation}\label{Equ: Actnorm}
    \hii = \sa \odot \hi + \biasa,
\end{equation}
where $\hi$ and $\hii$ are the intermediate latent representations during transformation. $\sa$ and $\biasa$ are the scale and translation parameters separately. $\odot$ is the dot product of tensors. The reverse operation of the Actnorm layer is
\begin{equation}\label{Equ: Actnorm}
    \hi = (\hii - \biasa) / \sa .
\end{equation}
$\sa$ and $\biasa$ are initialized to make each channel of the representations has zero mean and unit variance, like the normalization operation. However, different from the widely used normalization methods, during training, these parameters are updated through back propagation, without any constraints on the mean and variance of the latent variables any more. Employing the Actnorm layers is able to improve the training stability and performance. 

\textbf{Invertible $1\times1$ convolutional layers.} Different from the ordinary convolutional layers, the invertible $1\times1$ convolutional layers~\cite{Glow} we utilize here is designed for invertible normalizing flows and able to reverse. The operation in these layers can be represented as
\begin{equation}\label{Equ: Invertible}
    \hii = \textbf{W} \odot \hi,
\end{equation}
where $\textbf{W}$ is an square matrix which is initialized randomly.
Its reverse function is
\begin{equation}\label{Equ: Invertible}
    \hi = \textbf{W}^{-1} \odot \hii.
\end{equation}
These layers are to permute different channels of latent representaions.
% are generalizations of permutation operations employed in NICE~\cite{NICE} and Real NVP~\cite{RealNVP}

\textbf{Affine Coupling layers.} The Affine Coupling layers capture the correlations among spatial dimensions~\cite{NICE}~\cite{RealNVP}. The forward operations include:
\begin{gather*}\label{Equ: Affine Coupling_1}
    \hi^{a}, \hi^{b} = \text{Split}(\hi),  \\
    % \stwo, \biasb = \text{NN}(\hii^b), \\
    \hii^{a} = \hi^{a}+ \text{g}_1(\hi^b), \\ 
    \hii^{b} = \text{g}_2(\hii^a) \odot \hi^{b}+ \text{g}_3(\hii^a), \\ 
    \hii = \text{Concat}(\hii^{a}, \hii^{b}). 
\end{gather*}
where $\text{Split}(\cdot)$ and $\text{Concat}(\cdot)$ operate along channel dimensions. $\text{Split}(\cdot)$ splits $\hi$ to two tensors $\hi^{a}$ and $\hi^{b}$. $\text{Concat}(\cdot)$ concatenates two tensors $\hii^{a}$, $\hii^{b}$ along channel-wise to obtain $\hii$. $\text{g}_i(\cdot)$ ($i$=1, 2, 3) is neural network. The reverse operations are:
\begin{gather*}\label{Equ: Affine Coupling_1}
    \hii^{a}, \hii^{b} = \text{Split}(\hii),  \\
    \hi^{b} = (\hii^{b} - \text{g}_3(\hii^a))/\text{g}_2(\hii^a) , \\ 
    \hi^{a} = \hii^{a} - \text{g}_1(\hi^b), \\ 
    \hi = \text{Concat}(\hi^{a}, \hi^{b}). 
\end{gather*}
The operations in the second and third row turns $+$ into $-$ and $\odot$ into $/$. $\text{g}_i(\cdot)$ ($i$=1, 2, 3) can be any neural networks. Following~\cite{ardizzone2019guided} and~\cite{xiao2020invertible}, we employ Dense Block (DB) in our network as $\text{g}_i(\cdot)$.

\subsection{Objective Function}
Our objective function consists of two components, the distribution learning loss to encode the input noisy image $\y$ into latent code $\z$, and the reconstruction loss to restore corresponding clean image $\x$ with clean code $\zc$. The details of these two losses are as below.

\textbf{Distribution Learning Loss.}
\begin{equation}\label{loss:enc}
    L_{\text{dis}} = - \log p(\y) = - \big(\log p_{z}(\z)+\sum_{i=1}^{L} \log (\det|\frac{\partial f_{i}}{\partial \hi}|)\big)\;,
\end{equation}
where $L$ is the number of invertible layers in \ourmodel and $f_{i}$ is the function learned by each layer. $p_{z}(\z) \sim \ngaussian$ and $\z = (\zc, \zn)$.
To reconstruct the clean image, we set $\zn = \bm{0}$ and achieve a new latent representation $\hatz = (\zc, \bm{0})$, which lies in a subspace of $\z$.

\textbf{Reconstruction Loss.}
$\hatz$ is passed through the reverse network to restore the clean ground truth.
\begin{equation}\label{loss:rec}
    L_{\text{rec}} = ||f^{-1}(\hatz) - \x||_1\;.
\end{equation}

\textbf{Total Loss.} The total objective function we use during training is:
\begin{equation}
    L = \lambda_{1} L_{\text{dis}} + \lambda_{2} L_{\text{rec}}\;,
\end{equation}
where $\lambda_{1}$ and $\lambda_{2}$ are the weights for the two loss components.

% Our adjustment
% However,~\autoref{loss:enc} is non-convex, which is 

\begin{figure}[t]
\centering
% Caption
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\textwidth]{./secs/images/Crop.png} 
  \caption{Crop Methods}
  \label{subfig:crop}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\textwidth]{./secs/images/DataAugmentation3lines.png} 
  \caption{Data Augmentation}
  \label{subfig:augmentation}
\end{subfigure}
% \vspace{-2mm}
\caption{Comparisons on training with different processing strategies. (a) illustrates the difference between using random crop and center crop accompanied with resize. (b) shows the curves of validation results during training using different data augmentation methods. All the models are trained on CelebA~\cite{CelebA} with $\sigma=50$.}
% \vspace{-3mm}
\end{figure}

\subsection{Discussion of training details}
Since \ourmodel is the first distribution learning based denoising network, we explore different training strategies to demonstrate the way to make the best use of it.

\textbf{Random crop v.s. Center crop and resize.}
The widely used training strategy in feature learning based CNN denoising networks is to randomly crop patches from the training dataset to learn features. However, it is not so obvious whether the random crop strategy is also superior in distribution learning based networks. Take the face image denoising as an example, if we center crop the face region and resize it into an appropriate size, we will get a downscaled face image, which seems following similar distribution as the face image testset. Intuitively, the center crop with resize method will facilitate the network to learn the distribution better and achieve superior denoising results. 

Thus, we conduct the comparison on training with random crop and center crop with resize, illustrating the curves of the validation results on~\autoref{subfig:crop}. Contrary to our intuition, cropping training patches randomly outperforms the center crop with resize consistently and significantly.  
% potential reasons?
Therefore, we apply random crop during training \ourmodel.

\textbf{Data augmentation v.s. No data augmentation.}
Feature learning based networks usually employ horizontal and vertical flip and rotation with 90, 180, 270 degrees for data augmentation. However, these methods will bring in impossible patches, resulting in compromising the learning of distributions. For example, if we rotate a patch of face, we may get patches with the eyes under the mouth or on the left side of the mouth, which is impossible in face images. Although data augmentation introduces diverse features for feature learning methods having better generalization ability, it brings noise when learning the distributions.

We train three models for comparison: one with flip and rotation as data augmentation, one is only with flip as data augmentation and the other is trained without any augmentation. The validation results are shown in ~\autoref{subfig:augmentation}. The results verify our concern that inappropriate data augmentation such as rotation introduces noise to the distribution model, resulting in a lower denoising accuracy shown in the blue curve. Training with only flip as data augmentation achieves almost the same results as without data augmentation, but the latter one is more stable during training.
The potential reason might be that for face images, the horizontal flip also generates realistic images, while the vertical flip brings impossible face images, making the training unstable.
Thus, to avoid the unrealistic samples, we train our distribution learning based networks without data augmentation when the training set is large enough to learn the distribution. If the training set is small, we only conduct data augmentation which will not generate unrealistic patches.

% \begin{table*}[]
% \centering
% \caption{Comparisons of removing synthetic noise on three category-specific datasets. Our \ourmodel outperforms the other competitive methods on most of the three datasets for three different noise levels.} %In the meantime, \ourmodel ($1.46\times10^6$) has fewer parameters as compared to Unet ($7.70\times10^6$).
% \begin{tabular}{llcccccccccccc}
% \hline
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{BM3D} & \multicolumn{2}{c}{WNNM} & \multicolumn{2}{c}{DnCNN} & \multicolumn{2}{c}{FFDNet} &
% \multicolumn{2}{c}{GradNet} & \multicolumn{2}{c}{\ourmodel}\\ 
% \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{-2}{*}{$\sigma$}} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
% & 15  & 35.46 & & & & 31.47 & 0.9610 & 31.86 & 0.9577 & 31.58 & 0.9581 & \textbf{35.30} & \textbf{}  \\ % \textbf{32.50} & \textbf{0.9668} 
% & 25 & 32.80 & & & & 29.43 & 0.9466 & 28.94 & 0.9364  & 30.54 & 0.9548 & \textbf{32.95} & {}  \\ % {\bf 30.54} & {\bf 0.9557}
% \multirow{-3}{*}{CelebA~\cite{CelebA}} & 50 & 29.46 & & & & 26.71 & 0.9191 & 25.60 & 0.9060 & 27.68 & 0.9324  & \textbf{29.80} & \textbf{}  \\ \hline % \textbf{27.90} & \textbf{0.9353}
% % \multirow{-4}{*}{CelebA~\cite{CelebA}} & 70 & 27.92 & & & &  &  &  & &  &   & \textbf{28.27} & \textbf{}  \\ \hline % \textbf{27.90} & \textbf{0.9353}
% & 15 & 32.36 &  & & & 29.81 & 0.9561 & 30.88 & 0.9608 & 31.34 & 0.9648 & \textbf{32.08} & \textbf{0.9710}  \\ % BM3D 37.2029
% & 25 & 29.51 &  & & & 28.84 & 0.9492 & 28.27 & 0.9461 & 30.02 & 0.9580 & \textbf{30.31} & \textbf{0.9618} \\
% \multirow{-3}{*}{Flower~\cite{Flower}} & 50 & 26.03 &  & & & 26.11 & 0.9183 & 26.13 & 0.9238 & 26.99 & 0.9311 & \textbf{27.34} & \textbf{0.9379} \\ \hline
% % \multirow{-4}{*}{Flower~\cite{Flower}} & 70 & &  & & &  &  &  &  &  &  & \textbf{} & \textbf{} \\ \hline
% & 15 & &  & & & 30.08 & 0.9420 & 31.14 & 0.9470 & 31.79 & 0.9520 & \textbf{32.43} & \textbf{0.9589}  \\
% & 25 & &  & & & 28.49 & 0.9211 & 28.34 & 0.9284 & 29.37 & 0.9273 & \textbf{30.64} & \textbf{0.9453}  \\
% \multirow{-3}{*}{CUB-200~\cite{Bird}} & 50 & 26.42 &  & & & 26.45 & 0.8880 & 26.41 & 0.8993 & 27.65 & 0.9110 & \textbf{27.91} & \textbf{0.9171} \\ \hline
% % \multirow{-4}{*}{CUB-200~\cite{Bird}} & 70 & &  & & &  &  &  &  &  &  & \textbf{} & \textbf{} \\ \hline
% \end{tabular}
% \label{Tab:Class_Specific AWGN Denoise}
% \end{table*}


% \begin{table*}[]
% \centering
% \caption{Comparisons of removing synthetic noise on three category-specific datasets. Our \ourmodel outperforms the other competitive methods on most of the three datasets for three different noise levels.} %In the meantime, \ourmodel ($1.46\times10^6$) has fewer parameters as compared to Unet ($7.70\times10^6$).
% \begin{tabular}{llcccccccccc}
% \hline
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{BM3D} & \multicolumn{2}{c}{DnCNN} & \multicolumn{2}{c}{FFDNet} &
% \multicolumn{2}{c}{GradNet} & \multicolumn{2}{c}{\ourmodel}\\ 
% \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{-2}{*}{$\sigma$}} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
% & 15  & 33.27 & & 31.47 & 0.9610 & 31.86 & 0.9577 & 31.58 & 0.9581 & \textbf{35.21} & \textbf{}  \\ % \textbf{32.50} & \textbf{0.9668} 
% & 25 & 30.40 & & 29.43 & 0.9466 & 28.94 & 0.9364  & 30.54 & 0.9548 & \textbf{32.89} & {}  \\ % {\bf 30.54} & {\bf 0.9557}
% \multirow{-3}{*}{CelebA~\cite{CelebA}} & 50 & 26.67 & & 26.71 & 0.9191 & 25.60 & 0.9060 & 27.68 & 0.9324  & \textbf{29.75} & \textbf{}  \\ \hline % \textbf{27.90} & \textbf{0.9353}
% & 15 & & & 29.81 & 0.9561 & 30.88 & 0.9608 & 31.34 & 0.9648 & \textbf{32.08} & \textbf{0.9710}  \\
% & 25 & & & 28.84 & 0.9492 & 28.27 & 0.9461 & 30.02 & 0.9580 & \textbf{30.31} & \textbf{0.9618} \\
% \multirow{-3}{*}{Flower~\cite{Flower}} & 50 & & & 26.11 & 0.9183 & 26.13 & 0.9238 & 26.99 & 0.9311 & \textbf{27.34} & \textbf{0.9379} \\ \hline
% & 15 & & & 30.08 & 0.9420 & 31.14 & 0.9470 & 31.79 & 0.9520 & \textbf{32.43} & \textbf{0.9589}  \\
% & 25 & & & 28.49 & 0.9211 & 28.34 & 0.9284 & 29.37 & 0.9273 & \textbf{30.64} & \textbf{0.9453}  \\
% \multirow{-3}{*}{CUB-200~\cite{Bird}} & 50 & & & 26.45 & 0.8880 & 26.41 & 0.8993 & 27.65 & 0.9110 & \textbf{27.91} & \textbf{0.9171} \\ \hline
% \end{tabular}
% \label{Tab:Class_Specific AWGN Denoise}
% \end{table*}

% \begin{table*}[]
% \centering
% \begin{tabular}{llcccccccc}
% \hline
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{DnCNN} & \multicolumn{2}{c}{FFDNet} & \multicolumn{2}{c}{Unet} & \multicolumn{2}{c}{Glow}\\ 
% \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{-2}{*}{$\sigma$}} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
% & 15  & 31.47 & 0.9610 & 31.86 & 0.9577 & 31.77 & 0.9622 & \textbf{32.50} & \textbf{0.9668}  \\
% & 25 & 29.43 & 0.9466 & 28.94 & 0.9364 & \textbf{30.59} & \textbf{0.9563} & 30.54 & 0.9557  \\
% \multirow{-3}{*}{CelebA~\cite{CelebA}} & 50 & 26.71 & 0.9191 & 25.60 & 0.9060 & 26.48 & 0.9149  & \textbf{27.90} & \textbf{0.9353}  \\ \hline
% & 15 & 29.81 & 0.9561 & 30.88 & 0.9608 & 32.07 & \textbf{0.9715} & \textbf{32.08} & 0.9710  \\
% & 25 & 28.84 & 0.9492 & 28.27 & 0.9461 & 30.26 & \textbf{0.9620}& \textbf{30.31} & 0.9618 \\
% \multirow{-3}{*}{Flower~\cite{Flower}} & 50 & 26.11 & 0.9183 & 26.13 & 0.9238 & 27.17 & 0.9358 & \textbf{27.34} & \textbf{0.9379} \\ \hline
% & 15 & 30.08 & 0.9420 & 31.14 & 0.9470 & 31.96 & 0.9561 & \textbf{32.43} & \textbf{0.9589}  \\
% & 25 & 28.49 & 0.9211 & 28.34 & 0.9284 & 30.36 & 0.9432 & \textbf{30.64} & \textbf{0.9453}  \\
% \multirow{-3}{*}{CUB-200~\cite{Bird}} & 50 & 26.45 & 0.8880 & 26.41 & 0.8993 & 27.78 & 0.9167 & \textbf{27.91} & \textbf{0.9171} \\ \hline
% \end{tabular}
% \caption{Comparisons of removing synthetic noise on three category-specific datasets. Our \ourmodel outperforms the other three competitive methods on most of the three datasets for three different noise levels. Our model has fewer parameters as compared to Unet. }
% \label{Tab:Class_Specific AWGN Denoise}
% \end{table*}

% \begin{gather*}\label{Equ: Affine Coupling_1}
%     \hii^{a}, \hii^{b} = \text{split}(\hii),  \\
%     \stwo, \biasb = \text{NN}(\hii^b), \\
%     \hi^{a} = (\hii^{a} - \biasb)/\stwo, \\ 
%     \hi = \text{concat}(\hii^{a}, \hii^{b}).    
% \end{gather*}

% \begin{table}[]
% \centering
% \caption{The operations in the invertible module. In the inverse operations, only \textit{Plus} ($+$) becomes \textit{Minus} ($-$) and \textit{Multiply} ($\odot$) turns to \textit{Divide} ($/$). $\operatorname{\phi}_1$, $\operatorname{\phi}_2$, $\operatorname{\phi}_3$ and $\operatorname{\phi}_4$ do not need to be invertible. Thus, they can be any neural networks.}
% \vspace{-2mm}
% \renewcommand{\arraystretch}{1.6}
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{c|c}
% \hline
% \hline
% Forward & Backward \\ 
% \hline
% $\z^i_{a}$, $\z^i_{b} = \operatorname{Split}(\z^i)$ & $\z^{i+1}_{a}$, $\z^{i+1}_{b} = \operatorname{Split}(\z^{i+1})$ \\ \hline 
% $\z^{i+1}_{a} = \z^i_{a} \odot \operatorname{\phi}_1(\z^i_{b}) + \operatorname{\phi}_2(\z^i_{b})$ & $ \z^i_{a} = (\z^{i+1}_{a} - \operatorname{\phi}_2(\z^{i+1}_{b})) / 
% \operatorname{\phi}_1(\z^i_{b})$ \\ \hline
% $\z^{i+1}_b = \z^i_{b} \odot \operatorname{\phi}_3(\z^{i+1}_{a}) + \operatorname{\phi}_4(\z^{i+1}_{a})$ & $ \z^i_{b} = (\z^{i+1}_{b} - \operatorname{\phi}_4(\z^{i+1}_{a})) / \operatorname{\phi}_3(\z^i_{a})$ \\ \hline
% $\z^{i+1} = \operatorname{Concat}(\z^{i+1}_{a}, \z^{i+1}_{b})$ & $\z^i = \operatorname{Concat}(\z^i_{a}$, $\z^i_{b})$ \\ \hline
% % & &  \\ \hline
% \hline
% \end{tabular}
% }
% \vspace{-4mm}
% \label{Tab:Invertible_Module}
% \end{table}
% \renewcommand{\arraystretch}{1}

% In this paper, we explore employing similar components as~\cite{Glow} for image denoising by disentangling the latent variables in latent space. The network structure is shown in Figure~\ref{fig:NetArchi}, where the encoder and the decoder consist of $L$ levels of transformations and $K$ (inverse) flow steps for each level. 
% % Each Step of the Flow block contains an Actnorm layer, an Invertible $1 \times 1$ convolutional layer, and an Affine Coupling layer. 
% % Unlike Glow, 
% Our training can be divided into two stages: the encoding stage and the decoding stage. The encoding stage learns a series of multi-scale latent representations $\textbf{z}=(\textbf{z}_{0}, \cdots, \textbf{z}_{l}, \cdots,\textbf{z}_{L})$ for the input noisy images $\textbf{y}$ with the encoding loss $L_{enc}$,
% % We explored employing Glow for image denoising in this paper through disentangling the latent variables in latent space. The network structure is shown in Figure~\ref{fig:NetArchi}. Each Step of Flow block contains an Actnorm layer, an Invertible $1 \times 1$ convolutional layer and an Affine Coupling layer. Different from Glow, our training can be divided into two stages, \ie, the encode stage and the decode stage. The encode stage learns a series of multi-scale latent representations $\textbf{z}=(\textbf{z}_{0}, ..., \textbf{z}_{l},...,\textbf{z}_{L})$ for the input noisy images $\textbf{y}$ with the encode loss $L_{enc}$.
% % \begin{equation}\label{loss:enc}
% %     L_{enc} = - \log p(\textbf{y}) = - (\log p_{z}(\textbf{z})+\sum_{l=1}^{L} \log \det|\frac{\partial \textbf{f}_{l}}{\partial \textbf{h}_{l}}|)\;,
% % \end{equation}
% where $\textbf{h}_{l}$ is the internal variable we obtain during the transformation and $\textbf{z} \sim \textbf{N}(\textbf{0}, \textbf{I})$.

% Since $\textbf{z}$ follows the distribution $\textbf{N}(\textbf{0}, \textbf{I})$, the latent variables in each dimension are independent of each other. We assume that these latent variables can be disentangled into two parts, with some of the dimensions encoding the noise while the remaining dimensions encoding the clean images,  \ie, 
% $\textbf{z}_{noise}=(\textbf{z}_{n0}, \textbf{z}_{n1}, \cdots, \textbf{z}_{nL})$ and
% $\textbf{z}_{clean}=(\textbf{z}_{c0}, \textbf{z}_{c1}, \cdots, \textbf{z}_{cL})$. 
% Both of these two latent variables also follow the distribution $\textbf{N}(\textbf{0}, \textbf{I})$.
% In the decoding stage, we enforce $\textbf{z}_{noise}$ to be the mean of its distribution, \ie, the zero vector $\textbf{0}$, 
% % \SA{spell out 0 \ie zero} 
% and use $\textbf{z}_{clean}$ in the inverse process to restore clean images. A reconstruction loss $L_{rec}$ is employed to achieve the mentioned disentanglement:
% % \begin{equation}\label{loss:rec}
% %     L_{rec}(\bm{\theta}) = \frac{1}{N}\sum_{i=1}^{N} \frac{1}{2} ||\textbf{y}_i - \textbf{f}(\textbf{z}_{clean\_i})||_1\;.
% % \end{equation}


% \begin{comment}
% \begin{table*}[]
% \centering
% \caption{Comparisons of removing synthetic noise on three category-specific datasets. \ourmodel outperforms the other four competitive methods on most of the three datasets for three different noise levels. In the meantime, \ourmodel ($1.46\times10^6$) has fewer parameters as compared to Unet ($7.70\times10^6$).}
% \begin{tabular}{llcccccccccc}
% \hline
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{DnCNN} & \multicolumn{2}{c}{FFDNet} &
% \multicolumn{2}{c}{Unet} &
% \multicolumn{2}{c}{GradNet} & \multicolumn{2}{c}{\ourmodel}\\ 
% \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{-2}{*}{$\sigma$}} & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\ \hline
% & 15  & 31.47 & 0.9610 & 31.86 & 0.9577 & 31.77 & 0.9622 & 31.58 & 0.9581 & \textbf{32.50} & \textbf{0.9668}  \\
% & 25 & 29.43 & 0.9466 & 28.94 & 0.9364 & \textbf{30.59} & \textbf{0.9563} & 30.54 & 0.9548 & 30.54 & 0.9557  \\
% \multirow{-3}{*}{CelebA~\cite{CelebA}} & 50 & 26.71 & 0.9191 & 25.60 & 0.9060 & 26.48 & 0.9149 & 27.68 & 0.9324  & \textbf{27.90} & \textbf{0.9353}  \\ \hline
% & 15 & 29.81 & 0.9561 & 30.88 & 0.9608 & 32.07 & \textbf{0.9715} & 31.34 & 0.9648 & \textbf{32.08} & \textbf{0.9710}  \\
% & 25 & 28.84 & 0.9492 & 28.27 & 0.9461 & 30.26 & \textbf{0.9620} & 30.02 & 0.9580 & \textbf{30.31} & \textbf{0.9618} \\
% \multirow{-3}{*}{Flower~\cite{Flower}} & 50 & 26.11 & 0.9183 & 26.13 & 0.9238 & 27.17 & 0.9358 & 26.99 & 0.9311 & \textbf{27.34} & \textbf{0.9379} \\ \hline
% & 15 & 30.08 & 0.9420 & 31.14 & 0.9470 & 31.96 & 0.9561 & 31.79 & 0.9520 & \textbf{32.43} & \textbf{0.9589}  \\
% & 25 & 28.49 & 0.9211 & 28.34 & 0.9284 & 30.36 & 0.9432 & 29.37 & 0.9273 & \textbf{30.64} & \textbf{0.9453}  \\
% \multirow{-3}{*}{CUB-200~\cite{Bird}} & 50 & 26.45 & 0.8880 & 26.41 & 0.8993 & 27.78 & 0.9167 & 27.65 & 0.9110 & \textbf{27.91} & \textbf{0.9171} \\ \hline
% \end{tabular}
% \label{Tab:Class_Specific AWGN Denoise}
% \end{table*}
% \end{comment}

% Each Step of the Flow block contains an Actnorm layer, an Invertible $1 \times 1$ convolutional layer, and an Affine Coupling layer. In the sequel, we explain each of the layers.

% % \textbf{Actnorm layers} are layers with scale and translation parameters, performing affine transformations of the activations, as illustrated in Eq.~\eqref{Equ: Actnorm}. The parameters of these layers are initialized according to the input data to make each channel has zero mean and unit variance.
% % They are data-dependent initialized 
% % \SA{re-write} 
% % such that the post-actnorm activations per-channel has zero mean and unit variance. 
% % After initialization, they are trainable parameters during training 
% % \SA{re-write}. 
% Actnorm layers improve training stability and performance. The operation of these layers are denoted as:
% \begin{equation}\label{Equ: Actnorm}
%     \textbf{y} = \textbf{s} \odot \textbf{x} + \textbf{b}\;,
% \end{equation}
% where the scale parameters $\textbf{s}$ and bias $\textbf{b}$ are $1\times c$ scalars, and $c$ is the number of channels.

% \textbf{Invertible $1\times1$ convolutional layers} are generalizations of permutation operations employed in NICE~\cite{NICE} and Real NVP~\cite{RealNVP}, which is represented as
% \begin{equation}\label{Equ: Invertible}
%     \textbf{y} = \textbf{W}\textbf{x}\;,
% \end{equation}
% where $\textbf{W}$ is a $c \times c$ matrix.

% \textbf{Affine Coupling layers} capture the correlations among spatial dimensions, as in NICE~\cite{NICE} and Real NVP~\cite{RealNVP}. The operations they perform are listed below,
% \begin{equation}\label{Equ: Affine Coupling_1}
%     \textbf{x}_{a}, \textbf{x}_{b} = split(\textbf{x})\;, 
% \end{equation}
% \begin{equation}\label{Equ: Affine Coupling_2}
%     \textbf{s}_2, \textbf{b}_2 = NN(\textbf{x}_b)\;,
% \end{equation}
% \begin{equation} \label{Equ: Affine Coupling_3}
%     \textbf{y}_{a} = \textbf{s}_2 \cdot \textbf{x}_{a}+ \textbf{b}_2,\; \textbf{y} = concat(\textbf{y}_a, \textbf{x}_b)\;, \\    
% \end{equation}
% where $NN(\cdot)$ is a neural network, $split(\cdot)$ and $concat(\cdot)$ operate along channel dimensions.

% \SA{We have to re-write this section and combine it with the Background section. Before introducing glow, we have to talk about our method and then we move in the glow section without explicitly talking about glow as some reviewer might think that it is more about glow and we have no contribution in it.}

% \textbf{Discussion about adjusting $\lambda$.}
% Since the clean images are hard to get in reality, we treat the clean observations $\textbf{y}$ we got follows the distribution $\textbf{y} \sim N(\textbf{y}_{clean}, \sigma)$. $\sigma$ is a small margin. So the reconstruct loss can be written as Equation~\ref{equ: rec_loss_adjust}. With this training objective, we can learn the hyperparameter $\lambda_2$ during training automatically.

% \begin{equation} \label{equ: rec_loss_adjust}
%     L_{rec}(\theta) = \frac{1}{N}\sum_{i=1}^{N} \frac{1}{2 {\sigma}^2} ||y_i - f(z_i)||^2+\frac{1}{2}log {\sigma}^2
% \end{equation}

% \textbf{Discussion about the training and test image shape/distribution.}

% \textbf{Discussion about data augmentation v.s. no data augmentation.}


==> secs/RelatedWork_old.tex <==
\section{Related Work}
\subsection{Recent trends of image denoising}
\textbf{Traditional Methods.}
Traditional denoising methods usually construct an optimization scheme, modeling the distributions of noise or the priors of natural images as penalties or constraints.
The widely used natural image priors include sparsity~\cite{5459452}, total variation~\cite{TV}~\cite{2019_TV_multi_channel}, non-local similarity~\cite{1467423}~\cite{4154791} and external statistical prior~\cite{7410393}~\cite{6126278}.
NLM~\cite{1467423} computes a weighted average of non-local similar patches to denoise images. The weights are calculated by the Euclidean distance between pixels.
BM3D~\cite{BM3D} employs the structure similarity of patches in a transform domain, achieving excellent accuracy on denoising additive white gaussian noise (AWGN). 

However, most of the traditional methods are designed to tackle generic natural images. 
Very few work studies category-specific image denoising and considers the class specific priors while designing algorithms.
CSID~\cite{CSID} is the first to adopt external similar clean patches to facilitate denoising category-specific object images. They formulate an optimization problem using the priors in the transform domain. The objective consists of a Gaussian fidelity term that incorporates the category-specific information and a low-rank term that fortifies the similarity between noisy and external similar clean patches. They achieve superior denoising accuracy in removing noise from category-specific images.
Nonetheless, a common problem lies in most of these traditional model-driven methods is that it requires noise level as input. These methods usually put various hard thresholds to deal with different noise levels. However, the noise level is usually unavailable and we can only do blind denoising in reality, which limits the application of these methods.

\textbf{Deep learning Methods.}
Deep learning denoising methods learn models from a large amount of clean and noisy image pairs with CNNs, without providing image priors manually. Rapid progress of these methods has been seen in recent years, promoting the denoising effect significantly. The notable DnCNN~\cite{DnCNN} achieves good results on AWGN removing. After that, RIDNet~\cite{RIDNet} brings attention into denoising models, boosting the denoising performance further. VDN~\cite{VDN} makes assumptions on the distribution of clean images and noise, deriving a new evidence lower bound (ELBO) under the variational inference framework as the training objective. These CNN based denoising methods learn low-level features in the network to restore the details of clean images.

% category-specific image denoising
There are also few attempts in designing category-specific denoising networks recently. Remez etc.~\cite{8418389} propose a class-aware CNN based denoising method. They use a classifier to classify the noisy image into the supported classes first and then exploit the pretrained class-specific denoising models for denoising. For each of the supported classes, the denoising model is
pretrained on the images from the same classes of ImageNet~\cite{ILSVRC15}. The denoising architecture they proposed is a feature-learning based CNN.
However, for category-specific images, the feature learning based denoising methods usually impose the pixels of denoised images to be close to the clean ones but ignore the underlying distribution of the specific category. Thus, over-smoothed regions and artifacts are seen in restored images, degrading the visual effects of denoising. 
As far as we know, we are the first to conducted image denoising with distribution learning and disentanglement.

\subsection{Flow-Based Invertible Networks}
We employ normalizing flow based invertible neural networks to learn the distributions.
Normalizing flow~\cite{NICE} is a tool for computing complex distribution accurately. 
By applying a sequence of invertible transformations to transform a simple prior distribution to the complex distribution, the exact log-likelihood of the complex distribution can be computed. 

The key design concept of normalizing flow is invertibility, ensuring the mapping between an input and its output is one-to-one. Therefore, in order to estimate the probability density of image $\y$, we can alternatively achieve the same purpose via measuring the probability density of the counterpart latent variable $\z \sim \ngaussian$.
Estimating the probability density of $\y$ through using the probabilities of $\z$ requires taking the variations of metric spaces into consideration. Consequently, we have: 
\begin{equation}
        p(\y) =p(\z)\big|\det(\frac{\partial f^{-1}(\z)}{\partial \z})\big|
        =p(\z)\big|\det(\frac{\partial f(\z)}{\partial \z})\big|^{-1}, 
\label{Eq:density}
\end{equation}
where $\z = f(\y)$ and $\y = f^{-1}(\z)$. $f$ is the invertible function learned by normalizing flow. 

To reduce the complexity of computing the determinants of Jacobian matrices, special designs are applied in NICE~\cite{NICE} and Real NVP~\cite{RealNVP} to make each flow module has triangular Jacobian matrice. Glow~\cite{Glow} extends the channel permutation methods in these two models and proposes Invertible $1\times1$ convolutional layers. These models are usually used in image generation, demonstrating superior generation quality of natural images.

So far, few study applies invertible networks to image denoising.
Noise Flow~\cite{NoiseFlow} employs Glow~\cite{Glow} to learn the distribution of real-world noise and generate real noisy images for data augmentation. Extra information, such as raw images, ISO, and camera-specific parameters, is required during noisy image generation. 
Different from them, we are the first to exploit normalizing flow to learn the distribution of noisy images and disentangle the clean representations to restore images. In addition, we can also generate new noisy images by sampling noisy latent codes, without adding any extra information.
